Multi-Player Multi-Armed Bandits with Finite Shareable Resources Arms: Learning Algorithms & Applications

Multi-player multi-armed bandits (MMAB) study how decentralized players cooperatively play the same multi-armed bandit so as to maximize their total cumulative rewards. Existing MMAB models mostly assume when more than one player pulls the same arm, they either have a collision and obtain zero rewards, or have no collision and gain independent rewards, both of which are usually too restrictive in practical scenarios. In this paper, we propose an MMAB with shareable resources as an extension to the collision and non-collision settings. Each shareable arm has finite shareable resources and a "per-load" reward random variable, both of which are unknown to players. The reward from a shareable arm is equal to the "per-load" reward multiplied by the minimum between the number of players pulling the arm and the arm's maximal shareable resources. We consider two types of feedback: sharing demand information (SDI) and sharing demand awareness (SDA), each of which provides different signals of resource sharing. We design the DPE-SDI and SIC-SDA algorithms to address the shareable arm problem under these two cases of feedback respectively and prove that both algorithms have logarithmic regrets that are tight in the number of rounds. We conduct simulations to validate both algorithms' performance and show their utilities in wireless networking and edge computing.

==> sections/analysis.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Regret Analysis}

\subsection{Regret Analysis of \texttt{DPE-SDI}}
\begin{equation}
    \begin{split}
        \ERT \le & \!\sum_{k=L+1}^K\! \frac{(\mu_L -\mu_k)(\log T + 4 \log(\log T))}{\kl(\mu_k+\delta,\mu_L-\delta)} \\
            & + \sum_{k=1}^M \frac{16w_km_k^2}{\mu_k^2}\log T    \\
            & + 78M^2K^3(4+\delta^2) + 2Kh,
    \end{split}
\end{equation}
The largest per time slot expected reward of the optimal action $\bm{a}^*$ is
$
	\sum^{L-1}_{k=1} m_k \mu_k + (M-\sum_{k=1}^{L-1} m_k)\mu_L,
$
and the smallest reward of an action is $\min_{k\in[K]} m_k \mu_k$,
which happens when all $N$ plays are assigned to an arm with the smallest full load reward mean.
The largest per time slot regret denoted by $h$ is
\begin{equation*}
	h
	\coloneqq
	\sum^{L-1}\nolimits_{k=1} m_k \mu_k {+} \Big(M-\sum\nolimits_{k=1}^{L-1}m_k\Big)\mu_L - \min_{k\in[K]} m_k \mu_k.
\end{equation*}
For convenience, we denote $w_k$ as the cost upper bound of one round of IE and one round of UE for arm $k$,
$  w_k\coloneqq \Delta_{1,k}+\sum^{L-1}_{l=1} m_l \mu_l + (M-\sum_{l=1}^{L-1}m_l)\mu_L - m_k \mu_k.$


\subsection{Regret Analysis of \texttt{SIC-SDA}}
\begin{equation}
    \begin{split}
        \ERT \le  & c_1\sum_{k=L+1}^K \frac{m_k \log T}{\mu_L-\mu_k}  +  c_2\sum_{k=1}^M \frac{m_k^2}{\mu_k^2}\log T \\
        &+ c_3 K^2 \log^2\left(\min\left\{ \frac{\log (T)}{\mu_L - \mu_{L+1}}, T\right\}\right)        
    \end{split}
\end{equation}


DPE's analysis + TwoFold UCB's analysis Idea (decouple `learn capacities' and 'know capacities' parts).

To improve the constant term in DPE's upper bound, one can use the block setting~\cite{wang_optimal_2020}.

\begin{enumerate}
    \item Initialization: utilize  `share awareness', we show $\E[T_0] \le M^3  + M^2$.
    \item E-E phase: \begin{itemize}
        \item Exploration before learn optimal allocation: $2\times \E[\abs{\mathcal{A}\cup \mathcal{B}}]$ where $2$ is for both IE and UE. 
        \item Exploration during Exploitation: same as DPE $\sum_{k\ge L}(\mu_L - \mu_k)\E[\abs{\mathcal{G}_k}]$.
    \end{itemize} 
    \item Communication Phase: $6K \times M \times \E[\abs{\mathcal{A}}]$ where $6K$ is the number of rounds per phase (6 blocks), $M$ is the cost per round, $\E[\abs{\mathcal{A}}]\le \E[\abs{\mathcal{A}\cup\mathcal{B}}]$ is finite bounded.  
\end{enumerate}

==> sections/app_sic_sda.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Algorithmic Detail of \texttt{SIC-SDA}} \label{app:sic_sda}

\subsection{Initialization phase}\label{appsub:sic_sda_init}

\texttt{SIC-SDA}'s initialization phase (Algorithm~\ref{alg:sic_sda_init}) 
% is the same as~\cite{wang_optimal_2020}'s. 
% It 
consists of the orthogonalization and the rank assignment. 
The idea of orthogonalization is illustrated in \texttt{DPE-SDI}'s initialization phase (Appendix~\ref{appsub:dpe_sdi_init}), except that \texttt{SIC-SDA} needs to orthogonalize all players to \(K-1\) arms 
due to not knowing the number of players \(M\). 
After the orthogonalization steps, each player has a different external rank \(k\in [K-1]\). 
The rank assignment sub-phase aims to assign players with different ranks of \(\{1,2,\ldots,M\}\).
It takes \(2K-2\) consecutive time slots.
We number them as \(\{t_1, t_2, \ldots, t_{2K-2}\}\). 
During the rank assignment, players chooses arms according to the rule:
for player with external rank \(k\),
when \(t_s\in \{t_1,\ldots, t_{2k}\}\cup \{t_{K+k}, \ldots, t_{2K-2}\}\), he plays arm \(k\);
otherwise, when \(t_s \in \{t_{2k+1},\ldots, t_{K+k-1}\}\), he plays arm \(s-k\).
Following this rule, any pair of two players will share an arm exactly once. 
One can observe that the total number of sharing demand awareness in the first \(2k\) time slots plus one, i.e., \(\sum_{t\in\{t_1,\ldots, t_{2k}\}}\1{a_{k,t}>1}+1\), would become the arm's (internal) rank \(i\). 
The total number of sharing awareness in all \(2K-2\) time slots plus one, i.e., \(\sum_{t\in\{t_1,\ldots, t_{2K-2}\}}\1{a_{k,t}>1}+1\), is equal to the number of players \(M\). 

\begin{algorithm}[htp]
    \caption{\(\texttt{SIC-SDA.Init}()\)}
    \label{alg:sic_sda_init}
    \begin{algorithmic}[1]
        \State \algorithmicensure rank \(i\), the number of players \(M\)
        \State \(k \gets \text{Orthogonal}(K-1)\)
        \State \((i,M)\gets \text{RankAssign}(k)\) 
    \end{algorithmic}
\end{algorithm}

\subsection{Exploration phase}\label{appsub:sid_sda_explore}

Algorithm~\ref{alg:sic_sda_explore} illustrates the \texttt{SIC-SDA} algorithm's exploration phase. 
Its IE is in line~\ref{alg:sic_sda_explore:individual_explore_start}-\ref{alg:sic_sda_explore:individual_explore_end} and UE is in line~\ref{alg:sic_sda_explore:united_explore_start}-\ref{alg:sic_sda_explore:united_explore_end}.
Vector \(\bm{b}_t\in\N^K\) records how each active arm is shared in IE.
We note that IE and UE are phase-based: each arm is explored \(2^p\) times where \(p\) is the phase's index. 
%  according to line  the above rule. 
% The exploration phase's detail is deferred to Appendix~\ref{appsub:sid_sda_explore}.
% This is illustrated in Algorithm~\ref{alg:sic_sda_explore}'s line~\ref{alg:sic_sda_explore:individual_explore_start}-\ref{alg:sic_sda_explore:individual_explore_end} and Algorithm~\ref{alg:sic_sda_update}'s line~\ref{alg:sic_sda_update:b_start}-\ref{alg:sic_sda_update:b_end}.

\begin{algorithm}[htb]
    \caption{\(\texttt{SIC-SDA.Explore}(i, p,\bm{b}_t,\mathcal{K}_t, K_t, M_t)\)}
    \label{alg:sic_sda_explore}
    \begin{algorithmic}[1]
        \State \algorithmicensure \(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t\)
        \For{\(K_t2^p\) times} \Comment{Individual Exploration}\label{alg:sic_sda_explore:individual_explore_start}
            \If{\(i \le K_t\)}
                \State \(j\gets (i+t)\Mod{K_t}\)
                \State Play the \(j\)-th active arm.
                \State \(S^{\text{IE}}_{j,t}\gets S^{\text{IE}}_{j,t} + {r_{j,t}}/{b_{k,t}}\); \(\tau_{j,t}\gets \tau_{j,t}+1\) \label{alg:line:update_ie}
            \ElsIf{\(i > K_t\)}
                \State\multiline{Play the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n),t}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n),t}^l - 1)\) where \(\sigma(n)\) denotes the \(n\)-th active arm.}
            \EndIf
        \EndFor\label{alg:sic_sda_explore:individual_explore_end}
        \State \(\mathcal{K}'_t \gets \{k\in\mathcal{K}_t: m_{k,t}^l \neq m_{k,t}^u\}\)\label{alg:sic_sda_explore:united_explore_start}
        \For{\(2^p\) times} \Comment{United Exploration}
            \ForAll{ arm \(k \in \mathcal{K}'_t\)} 
                \State Play arm \(k\)
                \State \(S^{\text{UE}}_{k,t}\gets S^{\text{UE}}_{k,t} + r_{k,t}\); \(\iota_{k,t}\gets \iota_{k,t}+1\)
            \EndFor
        \EndFor\label{alg:sic_sda_explore:united_explore_end}
    \end{algorithmic}
\end{algorithm}
% \vspace{-10pt}

\subsection{Communication phase}\label{appsub:sic_sda_comm}

\begin{algorithm}
    \caption{\(\texttt{SIC-SDA.CommBack}(i, p, \bm{S}^{\text{IE}}_t)\)}
    \label{alg:sic_sda_commback}
    \begin{algorithmic}[1]
        \For{\((j,k)\in \{2,3, \ldots, \min\{M_t, K_t\}\}\times [K_t]\)}
            \If{\(i=1\)}
                \State \multiline{Leader receives \(S^{\text{IE}}_{k,t}(j)\) from follower with rank \(j\) in \(p+1\) time slots.} \label{alg:sic_sda_comback:line:leader_receive}
                \State \(S_{k,t}^{\text{IE}}(1) \gets S_{k,t}^{\text{IE}}(1) + S^{\text{IE}}_{k,t}(j)\)
                \State \(\tau_{k,t} \gets \tau_{k,t} + 2^p\)
            \ElsIf{\(i=j\)}
                \State \multiline{The follower with rank \(j\) sends \(S^{\text{IE}}_{k,t}(j)\) to leader in \(p+1\) time slots.} \label{alg:sic_sda_comback:line:follower_send}
            \EndIf 
        \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[htp]
    \caption{\texttt{SIC-SDA.CommForth}\((\mathcal{A}_t, \mathcal{R}_t, \bm{m}_t^l, \bm{m}_t^u)\)}
    \label{alg:sic_sda_commforth}
    \begin{algorithmic}[1]
        \For{Step \(s\in \{1,2,3,4,5\}\)} \Comment{1st-4th step}
            \For{\((k, j)\in \mathcal{K}_t \times [M_t]\)}
                \If{rank \(i=1\) } \Comment{leader}
                \If{\(s\)-th step's condition}\Comment{send signal}\label{alg:sic_sda_commforth:line:condition}
                    \State Play arm \(k\)-th active arm
                \Else\Comment{no update signal}
                    \State Play arm \((k+1)\Mod{K_t}\)-th active arm 
                \EndIf
                \ElsIf{rank \(i = j\)} \Comment{follower}
                    \State Play arm \(k\)-th active arm
                    \If{\(\1{a_{k,t} > 1} = 1\)} \Comment{detect signal}
                        \State \(s\)-th step's update \label{alg:sic_sda_commforth:line:update}
                    \EndIf
                \EndIf
            \EndFor
        \EndFor
    \end{algorithmic}
\end{algorithm}

The \(\texttt{SIC-SDA.CommBack}(i, p, \bm{S}^{\text{IE}}_t)\) is presented in Algorithm~\ref{alg:sic_sda_commback}. 
In the \(n\)-th phase, each arm is individually explored \(2^n\) times. 
So, a follower's accumulated reward of any arm till the end of phase \(p\) is at most \(2^{p+1} - 1\), and thus can be transmitted from the follower to leader in \(p+1\) time slots via the \(\1{a_{k,t} \ge 1}\) indicator, i.e., one time slot transmits one bit. 
The communication has a mesh-grid structure: for time slots corresponding to \((j,k)\in [2, \min\{M_t, K_t\}]\times [K_t]\), follower with rank \(i = j\) will send arm \(k\)'s IE reward summation \(S^{\text{IE}}_k\) to leader. 
We use \(S^{\text{IE}}_{k,t}(j)\) to indicate the accumulative IE rewards of the player with rank \(j\) when 
more than one players' \(S^{\text{IE}}_{k,t}\) appear simultaneously. 
%  in the same place. 
In line~\ref{alg:sic_sda_comback:line:leader_receive}'s \(p+1\) time slots, 
the leader always chooses arm \(1\). 
The received \(S^{\text{IE}}_{k,t}(j)\)'s binary expression's \(n\)-th position is \(1\) if the leader receives an arm sharing signal at the \(n\)-th time slot among the \(p+1\) slots, i.e., \(\1{a_{k,t}>1}=1\); 
and it is \(0\) otherwise. 
In line~\ref{alg:sic_sda_comback:line:follower_send}'s \(p+1\) time slots, 
the follower chooses arm \(1\) at the \(n\)-th time slot among the \(p+1\) slots if his \(S^{\text{IE}}_{k,t}(j)\)'s binary expression's \(n\)-th position is equal to \(1\), and chooses arm \(2\) otherwise.


The \texttt{SIC-SDA.CommForth}\((\mathcal{A}_t, \mathcal{R}_t, \bm{m}_t^l, \bm{m}_t^u)\) is illustrated in Algorithm~\ref{alg:sic_sda_commforth}. We present each step's condition (line~\ref{alg:sic_sda_commforth:line:condition}) and update (line~\ref{alg:sic_sda_commforth:line:update}) in Table~\ref{tab:sic_sda_comm_detail}. 


\begin{table}[htp]
    \centering
    \caption{\texttt{SIC-SDA.CommBack}'s details}
    \label{tab:sic_sda_comm_detail}
    \begin{tabular}{|c||c|c|}
        \hline
        Step & \(s\)-th step condition & \(s\)-th step update \\ \hline
        1st & \(k\in\mathcal{R}_t\) & \(\mathcal{K}_t \gets \mathcal{K}_t \setminus \{k\} \) \\
        2nd & \(k\in\mathcal{A}_t\) & \(\mathcal{K}_t \gets \mathcal{K}_t \cup \{k\} \) \\
        3rd & \(m_{k,t}^l > m_{k,\text{pre}}^l\) & \(m_{k,t}^l \gets m_{k,t}^l+1\) \\
        4th & \(m_{k,t}^u < m_{k,\text{pre}}^u\) & \(m_{k,t}^u \gets m_{k,t}^u - 1\) \\
        \hline
    \end{tabular}
\end{table}

% \subsection{Players Update Statistics}

\subsection{Successive accept and reject}~\label{appsub:sic_sda_sar}

In this subsection, we illustrate how leader accepts and rejects arms in the shareable arm setting, and how all players update their information after the leader's update. 

The successive accept and reject mechanism of \texttt{SIC-SDA} was made in~\cite{bubeck_multiple_2013} for top \(k\) arms identification and was utilized to design MMAB algorithms in~\cite{boursier_sic-mmab_2019}.
We further extend the idea to our \texttt{MMAB-SA} case where accepting and rejecting arms not only depends on arm's reward means, but also on theirs shareable resources which are unknown a prior.

\setlength{\textfloatsep}{0pt}
\begin{algorithm}[htp]
    \caption{\(\texttt{SIC-SDA.AccRej}(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t, \mathcal{K}_t, M_t)\)}
    \label{alg:sic_sda_accept_and_reject}
    \begin{algorithmic}[1]
        \State \algorithmicensure \(\mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t,\bm{m}_t^l, \bm{m}_t^u\)
        \If{\(i=1\)}
            \State \(\hat{\mu}_{k,t}\gets {S}_{k,t}^{\text{IE}} / {\tau}_{k,t}, \hat{\nu}_t\gets {S}_{k,t}^{\text{UE}} / {\iota}_{k,t},\,\forall k\)
            \State Update \(\bm{m}^l_t, \bm{m}^u_t\) according to Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update})
            \State \multiline{Update \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t\) by Eq.(\ref{eq:accept_set})(\ref{eq:reject_set})(\ref{eq:marginal_arm})}
        \EndIf
    \end{algorithmic}
\end{algorithm}

\noindent
\textbf{Leader accepts and rejects arms.} After leader receives followers' IE observations, 
the leader updates his empirical reward mean and check whether there are some optimal (sub-optimal) arms that should be accepted (rejected). 
Denote \(g(k,j)\) as a special indicator function for distinguishing ``good'' arm \(k\) from ``bad'' arm \(j\) as follows
\[g(k,j)\coloneqq \1{\hat{\mu}_{k,t}- 3\sqrt{\frac{\log (T)}{2\tau_{k,t}}}\ge \hat{\mu}_{j,t}+  3\sqrt{\frac{\log (T)}{2\tau_{j,t}}}},\] 
where $g(k,j) =1$ implies that the arm \(k\)'s reward mean is higher than arm \(j\)'s with high confidence.
% For an arm \(k\), denote \(\mathcal{B}_{k,t} \coloneqq \{i\in\mathcal{K}_t: g(k,i)=0\}\) as  

The leader accepts arm \(k\) if  the arm's resources are well estimated, i.e., \(k\in\mathcal{K}_t\setminus \mathcal{K}'_t\) and \(
    \sum_{j\in\mathcal{K}_t: g(k,j) = 0} m_{j,t}^u \le M_t
\), which means the total resources' upper confidence bounds 
of arms which cannot be distinguished as bad by arm \(k\) (i.e., \(g(k,j) = 0\)) is no greater than the number of active players \(M_t\).
Thus, the accept arm set \(\mathcal{A}_t\) can be set as:
\begin{equation}\label{eq:accept_set}
    \mathcal{A}_t \coloneqq \left\{k\in\mathcal{K}_t\setminus \mathcal{K}'_t:   \sum\nolimits_{j\in\mathcal{K}_t: g(k,j) = 0}  m_{j,t}^u \le M_t\right\}. 
\end{equation}
The leader rejects arm \(k\), if \(
    \sum_{j\in\mathcal{K}_t: g(j,k) = 1} m_{j,t}^l \ge M_t 
\). 
The inequality means that the total resources' lower confidence bounds of arms whose reward mean is higher than arm \(k\)'s with high confidence (i.e., \(g(j,k) = 1\)) is no less than \(M_t\).
Thus, the reject arm set \(\mathcal{R}_t\) can be expressed as:
\begin{equation}\label{eq:reject_set}
    \mathcal{R}_t \coloneqq \left\{k\in\mathcal{K}_t: \sum\nolimits_{j\in\mathcal{K}_t: g(j,k) = 1} m_{j,t}^l \ge M_t\right\}. 
\end{equation}
An arm \(k\) is the empirical least favored among optimal arms if its empirical reward mean is higher than all other current active arms' with high confidence (i.e., the only optimal arm among them), and its resources' lower confidence bound is no less than \(M_t\), i.e.,
% \(
%     \sum_{i\in\mathcal{K}_t} g(k,i) = \abs{\mathcal{K}_t} - 1 \text{ and } m_k^l \ge M_t.
% \)
% The marginal accept arm \(\mathcal{L}_t\) corresponds to the worst arm among optimal arms and the ``marginal'' means the arms' capacity may only be marginally utilized.   
\begin{equation}\label{eq:marginal_arm}
    \mathcal{L}_t\! \coloneqq \!\left\{k\in\mathcal{K}_t \! : \!\! \sum\nolimits_{j\in\mathcal{K}_t} \! g(k,j)\! = \! K_t\! - \!1, m_{k,t}^l \!\ge\! M_t \right\}.
\end{equation}


\subsection{Update Players' status. }~\label{appsub:sic_sda_update}
After the leader sends back his updated information to followers, all players update their status according to Algorithm~\ref{alg:sic_sda_update}.
It consists of three steps: (1) upon finding the least favored arm,
(line~\ref{alg:line:sic_sda_update_least_favored_arm}), 
all active players turn to exploit this arm,
(2) if there are accepted arms,
(line~\ref{alg:line:sic_sda_update_accepted_arm}), 
several players will turn to exploit these arm, and the number of players exploiting an arm is equal to the arm's resources capacity,
% their resources size \(m_k\) number of players turns to exploit them,
and (3) if  \(M_t > K_t\) (line~\ref{alg:line:sic_sda_update_b} ), update the vector \(\bm{b}_t\) to record the player allocation in the next IE round. 
% Their details are deferred to Appendix~\ref{appsub:sic_sda_update}.

\begin{algorithm}[htp]
    \caption{\(\texttt{SIC-SDA.Update}(i, \mathcal{K}_t, M_t, \mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t)\)}
    \label{alg:sic_sda_update}
    \begin{algorithmic}[1]
        \State \algorithmicensure \(\text{ExploitArm}, \mathcal{K}_t, M_t\)
        \State \(M_t \gets M_t - \sum_{k\in\mathcal{A}_t}m_{k,t}^l\)
        \State \(\mathcal{K}_t \gets \mathcal{K}_t\setminus (\mathcal{A}_t \cup \mathcal{R}_t \cup \mathcal{L}_t)\)

        \If{\(\mathcal{L}_t \neq \emptyset\)}\label{alg:line:sic_sda_update_least_favored_arm}\Comment{exploit the leader favored arm}
            \State  \(\text{ExploitArm}\gets \mathcal{L}_t.\)
        \ElsIf{\(i > M_t\)}\label{alg:line:sic_sda_update_accepted_arm}\Comment{exploit accepted arm}
            \State \multiline{\(\text{ExploitArm}\gets j\)-th accept arm where such that \(\sum_{n=1}^j m_{\sigma'(n),t}^l \ge i-M_t > \sum_{n=1}^{j-1} m_{\sigma'(n),t}^l\) where \(\sigma'(n)\) is the \(n\)-th accept arm.}
        \Else 
            \State \(\bm{b}_t\gets \bm{1}.\) \Comment{update player allocation in next IE} \label{alg:sic_sda_update:b_start}
            \If{\(M_t > K_t\)}\label{alg:line:sic_sda_update_b} 
                \State \(d\gets M_t - \abs{\mathcal{K}_t}.\)
                \ForAll{\(k \in \mathcal{K}_t\)}
                \While{\(d>0\) and \(b_{k,t} < m_{k,t}^l\)}
                    \State \(b_{k,t} \gets b_{k,t} + 1\); \(d\gets d - 1\).
                \EndWhile
                \EndFor
            \EndIf \label{alg:sic_sda_update:b_end}
        \EndIf
        \State \(p\gets p + 1\)  
    \end{algorithmic}
\end{algorithm}

==> sections/dpe_sa_algo_backup.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Decentralized Parsimonious Exploration for Sharing Demand Information Feedback}



In this section, we propose the \texttt{DPE-SDI} algorithm solving the sharing information feedback setting.
\texttt{DPE-SDI} employs a leader-follower structure: choose one player as the leader, and assign the rest \(M-1\) players as followers. 
The leader takes the responsibility of collecting observations and updating empirical optimal arms to followers. 
The followers don't need to communicate anything to the leader.
\texttt{DPE-SDI} consists of three main phases: 
\begin{enumerate}
    \item Initialization phase: estimate the total number of players \(M\) and assign ranks to all players. \begin{itemize}
        \item Player with rank \(1\) becomes the leader. 
    \end{itemize}
    \item Exploration-Exploitation phase: \begin{itemize}
        \item Exploitation: followers exploit empirical optimal arms. 
        \item Parsimonious exploration: the leader parsimoniously explore empirical sub-optimal arms.  
        \item United exploration: all players rally to explore some empirical optimal arms whose capacities have not be well estimated. 
    \end{itemize}
    \item Communication phase: When the leader needs to update his decision and knowledge, he initializes a round of communication and send them to followers.
\end{enumerate}

Denote \(\hatbm{a}^*(t) \coloneqq (\hat{a}_1^*(t), \ldots, \hat{a}_K^*(t))\) as the empirical optimal assignment profile according to observations up to time \(t\). 
Denote the empirical optimal arm set as \(\mathcal{S}(t)\coloneqq \{k: \hat{a}_k^*(t) > 0\}\)
and the empirical least favored arm among empirical optimal arms as \(\mathcal{L}(t)\).
Note that the leader does not need to transmit the empirical optimal action \(\hatbm{a}_k^*(t)\in \N^K\) to its followers, which might take plenty of steps for communication in one update. 
Because followers can recover \(\hatbm{a}^*(t)\) from \(\mathcal{S}(t), \mathcal{L}(t), \bm{m}^l(t)\): 
for arms \(k\) in \(\mathcal{S}(t)\) but not \(\mathcal{L}(t)\), the \(\hat{a}_k^*(t)\) is equal to \(m_k^l(t)\);
while the\(\hat{a}_{\mathcal{L}(t)}^*(t)\) of the empirical least favored arm is equal to \(M - \sum_{k\in\mathcal{S}(t), k\neq \mathcal{L}(t)} m_k^l\).

% We note that the leader only makes use of his onw observations and send his decision, i.e., \(\mathcal{S}, L(t), \bm{a}(t), \bm{m}^l, \bm{m}^u\), to followers. 



% For the easy of illustration, we give a simplified framework in Algorithm~\ref{alg:dpe_adapt}. 
% To achieve the optimal regret bound in our analysis, one needs to introduce a block-based communication scheme in which leader can only start a communication round at the beginning of a block. 

\begin{algorithm}[htp]
    \caption{\texttt{DPE-SDI}}
    \label{alg:dpe_adapt}
    \begin{algorithmic}[1]
        \State \LeftComment{Initialization Phase}
        \State Initialization: \(i, L, M\gets 0, \quad \mathcal{S}, \mathcal{S}'\gets \emptyset,\quad  \bm{m}^{l},\bm{m}^{u}\gets (1,\ldots,1)^T, \quad \hatbm{\mu},\hatbm{u}\gets (0,\ldots,0)^T\)
        \State \(M \gets\text{Rally}.\) \label{algline:rally}
        \State \(i\gets \text{Orthogonal}(M).\) \label{algline:rankassignment}
        
        \While{\(t\le T\)}
        \State \LeftComment{Exploration-Exploitation Phase: } Algorithm~\ref{alg:DPE-SDI-exploration}
        % \State \textsc{Parsimonious and United Exploration} (Algorithm~\ref{alg:DPE-SDI-exploration})
        \State Leader updates statistics: Algorithm~\ref{alg:DPE-SDI-update-stats}
        \State \LeftComment{Communication Phase}
        \If{any of \(\mathcal{S}(t),L(t),\bm{m}^{l}(t), \bm{m}^{u}(t)\) changes}
        \State Leader sends these information to followers
        \State \(t\gets t+ C\)
        \EndIf
        \EndWhile
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[htp]
    \caption{Leader Updates Statistics}
    \label{alg:DPE-SDI-update-stats}
    \begin{algorithmic}[1]
        \If{\(i=1\)}
            \State \(\hat{\mu}_k(t)\gets {S}_k^{\text{IE}}(t) / {\tau}_k(t), \hat{\nu}(t)\gets {S}_k^{\text{UE}}(t) / {\iota}_k(t),\,\forall k\)
            \State Updates \(\bm{m}^{l}(t), \bm{m}^{u}(t)\) via Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update})
            \State{\(\hatbm{a}^*(t)\gets \Oracle(\hat{\bm{\mu}}(t), \bm{m}^l(t))\)}
            \State{\(\mathcal{S}(t)\gets \{k: \hat{a}_k^*(t) > 0\}\)}
            \State{\(\mathcal{L}(t)\gets \argmin_k\{\hat{\mu}_{k}:a_{k}(t) > 0\}\)}
            \State{$\mathcal{E}(t)\gets \{k: u_k(t) \ge \hat{\mu}_{L(t)}(t), a_{k}(t) = 0\}.$}
        \EndIf
    \end{algorithmic}
\end{algorithm}




\subsection{Initialization Phase}

The initialization phase contains two parts: probing the total number of players \(M\) (Rally in line~\ref{algline:rally}), and assigning each player a rank from \(\{1,2,\ldots, M\}\) (Orthogonal in line~\ref{algline:rankassignment}). 

For Rally at the first time slot, all players just choose arm 1 (or any other pre-determined arm). Then from SDI $a_1(1)$, all players would observe the total number of players \(M\). 

We employ an orthogonalization approach to assign ranks that is similar to \cite{wang_optimal_2020}'s. 
% As the number of players \(M\) is known, we can apply a randomized orthogonalization. 
Each player starts with a rank \(M+1\).
The algorithm runs in rounds and each round contains \(M+1\) time slots. 
In the beginning of a round, if the player's rank is \(M+1\), then he uniformly choose an arm \(i\in [M]\) to play,
and if its rank \(i\) is less than \(M+1\), he plays arm \(i\).
If player with rank \(M+1\) receives the feedback \(a_j(t) = 1\), he updates his rank to \(j\);
otherwise, there are other players sharing the arm and his rank is still \(M+1\). 
In the round's subsequent \(M\) time slots, each player always chooses their rank's corresponding arm 
except that at the \((i+1)\)th time slot she chooses arm \(M+1\). 
If each player was orthogonally assigned with a rank in \(\{1,2,\ldots,M\}\), in these subsequent \(M\) time slots, no sharing (i.e., \(a_k(t) > 1\)) would happen. Or otherwise, all players will experience arm sharing at least once. 
We show the expected time slots of this orthogonalization is \(\E[T_0]\le M^3+M^2\) in Appendix~\ref{appsub:dpe_sa_init}.

% \textbf{Appendix.} give the \(\E[T_0]\) analysis. 

This initialization procedure is different from the common one of MMAB: first assign external ranks via orthogonalization, and then assign internal rank and estimate \(M\) via sequential hopping, e.g., in DPE1~\cite{wang_optimal_2020} and SIC-MMAB~\cite{boursier_sic-mmab_2019}. 
Our initialization phase is much simpler than the common one, thanks to the SDI feedback. 
From this feedback, players can easily observe the number of players \(M\). 
Knowing \(M\), one just need to orthogonalize \(M\) players to \(M\) arms and the player's orthogonalized arm index can be used as its internal rank directly. 

\subsection{The Exploration-Exploitation Phase}

\begin{algorithm}[htp]
    \caption{Exploration-Exploitation Phase}
    \label{alg:DPE-SDI-exploration}
    \begin{algorithmic}[1]
        \For{\(M\) times} \Comment{Parsimonious exploration}
            \State \multiline{Find \(j\) such that  \(\sum_{i=1}^{j} a_j(t) \ge (i+t)\Mod{M} > \sum_{i=1}^{j-1} a_j(t)\)}
            \If{\(i\neq 1\)}\Comment{Follower}
                \State{Play arm \(j\)} 
            \ElsIf{\(i=1\)}\Comment{Leader}
                \If{\(\mathcal{E}(t) \neq \emptyset\) and \(j = L(t)\)}
                    \State{w.p. $1/2$, \(k\gets l\sim\mathcal{E}(t)\) uniformly}
                    \State{w.p. $1/2$,  \(k\gets j\)}
                \Else 
                    \State{ \(k\gets j\)}
                \EndIf
                \State Play arm \(k\)
                \State \(S^{\text{IE}}_k(t) \gets S^{\text{IE}}_k(t)  + \frac{r_k(t)}{a_k(t)}, \tau_k(t)\gets \tau_k(t) + 1\)
            \EndIf
            \State \(t\gets t+1\).
        \EndFor

        \State \(\mathcal{K}'(t)\gets \{k\in\mathcal{K}(P): m_k^{l} \neq m_k^{u}\}.\)
        \For{\(k\in\mathcal{K}'(t)\)}
            \State All players choose arm \(k.\) \Comment{United exploration}
            \State \(S^{\text{UE}}_k(t) \gets S^{\text{UE}}_k(t)  + r_k(t)\)
            \State \(\iota_k(t) \gets \iota_k(t) + 1, t\gets t+1\).
        \EndFor
    \end{algorithmic}
\end{algorithm}

\textbf{Parsimonious exploration.} 
All players play the empirical optimal assignment profile \(\hatbm{a}^*(t)\) and they rotate over the empirical optimal arms in different time slots. 
Specifically, given \(\hatbm{a}^*(t)\), the player with rank \(i\) plays arm \(j\) such that \(\sum_{i=1}^{j} a_j(t) \ge (i+t)\Mod{M} > \sum_{i=1}^{j-1} a_j(t)\).
Only when the leader plays the empirical least favored arm can she 
explore an empirical sub-optimal arm with a  $0.5$ probability if the arm's KL-UCB index~\cite{cappe_kullback-leibler_2013} is larger than the empirical least favored arm's. Denote $u_k(t)$ as the KL-UCB index as follows:
\[
    u_k(t) = \sup\{q\ge 0: \tau_{k}(t)\kl(\hat{\mu}_{k}(t), q)\le f(t)\},
\]
where $f(t) = \log (t) + 4 \log\log(t)$, $\tau_{k}(t)$ denote the number of explorations for arm $k$ up to time $t$. 
We denote \(\mathcal{E}(t)\) as a subset of empirical sub-optimal arms whose KL-UCB index is larger than the least favored arm \(\mathcal{L}(t)\)'s, i.e., \(\mathcal{E}(t)\gets \{k: u_k(t) \ge \hat{\mu}_{L(t)}(t), a_{k}(t) = 0\}.\)
We note that the parsimonious exploration idea was first made in~\cite{combes_learning_2015} for learning-to-rank algorithm and was further utilized in~\cite{wang_optimal_2020} for multiple player setting. 

\textbf{United exploration.}
UE refers to all \(M\) players rallying on an arm so that they can observe a sample of reward random variable when its resources are fully utilized \(m_kX_k\). 
Collecting this kind of observation is crucial in estimating an arm's shareable resources \(m_k\) (see next subsection).
Arm set \(\mathcal{S}'(t)=\{k:a_k(t) > 0, m_k^{l}(t) \neq m_k^{u}(t)\}\) contains empirical optimal arms whose amount of resources have not been learnt.
In one round of exploration-exploitation phase, all \(M\) players rally to each arm of \(\mathcal{S}'(t)\) once in turn.
%  in \(\abs{\mathcal{S}'}\) time slots.
Denote \(S_k^{\text{UE}}(t)\) as the total reward of UE from arm \(k\) up to time \(t\), \(\iota_k(t)\) as the number of UE times for arm \(k\) up to time \(t\), and the empirical mean estimate of \(\E[m_kX_k]\) is \(\hat{\nu}_k(t)\coloneqq S_k^{\text{UE}}(t) / \iota_k(t)\).


\subsection{Confidence Bounds of Shareable Resources}
In this subsection, we provide a method to construct upper and lower confidence bound of shareable resources. 

\textbf{Individual exploration.} As a contrast to united exploration (UE), we define another type of exploration called individual exploration (IE) when one assures \(a_k(t) < m_k\).
The simplest case of IE happens when an individual player chooses arm \(k\),
but it also includes cases that several players share an arm.
For example, we note the leader's actions during parsimonious exploration can all be regarded as IEs.
So, divided by \(a_k(t)\), IE's rewards can be employed to estimate the reward mean \(\hat{\mu}_k(t) = \bm{S}_k^{\text{IE}}(t)/\tau_k(t)\), where \(\bm{S}_k^{\text{IE}}(t)\) is the summation of IE's reward feedback (divided by the number of players on arm \(k\)) up to time slot \(t\) and \(\tau_k(t)\) is the number of IE times for arm \(k\) up to time slot \(t\).
% We note that the leader's actions during parsimonious exploration can  

% Utilize the capacity estimator and uniform confidence interval;

\begin{lemma}[Confidence interval for shareable resources $m_k$]\label{lma:confidence_bound}
    Denote the function
    \(
        \phi(x,\delta) \coloneqq \sqrt{\left(1+\frac{1}{x}\right)\frac{\log(2\sqrt{x+1}/\delta)}{2x}}.
    \)
    When $\phi(\tau_{k}(t),\delta) + \phi(\iota_{k}(t),\delta) < \hat{\mu}_{k}(t)$, the event
    \begin{align}
        &\bigg\{\!\forall \tau_{k}(t), \iota_{k}(t) \!\in\!\mathbb{N}_+,
        m_k \!\in\! 
        \bigg[\frac{\hat{\nu}_{k}(t)}{\hat{\mu}_{k}(t) + \phi(\tau_{k}(t),\delta) + \phi(\iota_{k}(t),\delta)}, \nonumber \\
        &\qquad\qquad\qquad \frac{\hat{\nu}_{k,t}}{\hat{\mu}_{k}(t) - \phi(\tau_{k}(t),\delta) - \phi(\iota_{k}(t),\delta)}\bigg] \bigg\}\label{eq:confidence_bound}
    \end{align}
    holds with a probability of at least $1-\delta$.
\end{lemma}


% \begin{lemma}[Resources \(m_k\) Estimation Criterion (cite the centralized paper)]\label{lma:confidence_bound}
%     Denote \(\phi(x,\delta)\coloneqq \sqrt{\left( 1+\frac 1 x \right) \frac{\log(2\sqrt{x+1}/\delta)}{2x}}\) and assume 
%     \(\phi(\tau_k(t), \delta) + \phi(\iota_k(t), \delta) < \hat{\mu}_k(t)\).
%     For any arm \(k\), if 
%     \begin{equation}\label{eq:estimation_criterion}
%         \begin{split}
%         &\ceil{\frac{\hat{\nu}_k(t)}{\hat{\mu}_k(t) + \phi(\tau_k(t), \delta) + \phi(\iota_k(t), \delta)}} \\
%         = &
%         \floor{\frac{\hat{\nu}_k(t)}{\hat{\mu}_k(t) - \phi(\tau_k(t), \delta) - \phi(\iota_k(t), \delta)}},            
%         \end{split}
%     \end{equation}
%     then the probability of correctly estimating \(m_k\) is at least \(1-\delta\), i.e., \(\P(\hat{m}_k(t) = m_k)\ge 1-\delta\).
% \end{lemma}

From Lemma~\ref{lma:confidence_bound}, we can calculate the shareable resources \(m_k\)'s lower and upper confidence bounds as follows:
\begin{align}
    & m_k^l(t) = \label{eq:lower_bound_update}\\
    &\max\left\{m_k^l(t-1), \ceil{\frac{\hat{\nu}_k(t)}{\hat{\mu}_k(t) + \phi(\tau_k(t), \delta) + \phi(\iota_k(t), \delta)}}\right\},\nonumber\\
    &m_k^u(t) = \label{eq:upper_bound_update}\\
    & \min\left\{m_k^u(t-1), \floor{\frac{\hat{\nu}_k(t)}{\hat{\mu}_k(t) - \phi(\tau_k(t), \delta) - \phi(\iota_k(t), \delta)}}\right\}.\nonumber
\end{align}



\subsection{Leader-Follower Communication Protocol}

% the leader sends the empirical optimal arm set \(\mathcal{S}\), the minimal empirical mean arm \(\mathcal{L}\), and the confidence lower bounds \(\bm{m}^l\) to follower, 

After each round of the exploration-exploitation phase, the leader updates its information. 
If there are any changes of \(\mathcal{S}(t), \mathcal{L}(t),\bm{m}^{l}(t), \bm{m}^{u}(t)\), 
leader will initialize a round of communication to update these information of followers. 
For simplicity, we illustrate the communication as 6 sub-blocks as follows. 
Some potential improvements of the communication is discussed in Appendix~\ref{appsub:dpe_sa_comm}.

\begin{enumerate}
	\item Initial block: the leader signifies followers to start communication. 
	\item Second block: notify a subset of arms to be removed from \(\mathcal{S}(t)\).
	\item Third block: notify a subset of arms to be added in \(\mathcal{S}(t)\). 
	\item Forth block: notify the empirical least favored arm \(\mathcal{L}(t)\) among \(\mathcal{S}(t)\).
	\item Fifth phase: update capacities' lower bound \(\hatbm{m}^l\).
	\item Sixth phase: update capacities' upper bound \(\hatbm{m}^u\).
\end{enumerate}

\emph{Initial block:} 
When the leader needs to update followers' information after an exploration-exploitation phase, 
he stops at the arm \(\hat{k}^*\) with highest estimate mean.
Followers start the next round's exploration-exploitation phase (i.e., play arms of \(\hatbm{a}^*(t)\) in turn). 
In subsequent time slots, followers playing arm \(\hat{k}^*\) would observe \(a_{k^*}(t) > m_{k^*}^l\),
which violates the profile \(\hatbm{a}^*(t)\),
and realize that a communication starts. 
We note that this ad-hoc communication initialization is crucial for \texttt{DPE-SDI} and when considering weaker SDA feedback, such ad-hoc communication is invalid.

In the remaining 5 blocks, 
followers cooperate to play same arms and rotate over all \(K\) arms once in each block.
% all followers always play the same arm and play all \(K\) arms in turn.
Each block is exactly \(K\) time slots. 
When these followers are on an arm \(k\), the number of players sharing arm \(k\) is at least \(M-1\), i.e., \(a_k(t) \ge M-1\). 
When the leader wants to update information related to arm \(k\) in some blocks, she will choose arm \(k\) when followers play the arm. So that all followers observe \(a_k(t) = M\), which is a signal for updating arm \(k\)'s related information.

For these 5 blocks, the \(a_k(t) = M\) signal respectively stands for 
removing arm \(k\) from estimated optimal arm set \(\mathcal{S}(t)\) (2nd),
adding arm \(k\) to \(\mathcal{S}(t)\) (3rd),
updating arm \(k\) as the empirical least favored arm \(\mathcal{L}(t)\) (4th),
increasing arm \(k\)'s capacity lower bound \(m_k^l\) by 1 (5th), and 
decreasing arm \(k\)'s capacity upper bound \(m_k^u\) by 1 (6th).

% \subsection{Regret Analysis}
% \subsubsection{RegA}





==> sections/dpe_sdi_algo_backup.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Decentralized Parsimonious Exploration for Sharing Demand Information Feedback}

In this section, we propose the \texttt{DPE-SDI} algorithm solving the sharing information feedback setting.

\subsection{Overview of The Design}

Algorithm \ref{alg:dpe_sdi} outline the \texttt{DPE-SDI} algorithm.   
The \texttt{DPE-SDI} employs a leader-follower structure: 
choose one player as the leader, and assign the rest \(M-1\) players as followers. 
The leader takes the responsibility of collecting observations and updating empirical optimal arms to followers. 
Followers don't need to communicate anything to the leader.
\texttt{DPE-SDI} consists of three main phases: 
\textit{initialization phase}, 
\textit{exploration-exploitation phase} 
and \textit{communication phase}.  
The \textit{initialization phase} (Line \ref{algo:SDI-init}) 
estimates the total number of players 
\(M\) and assign ranks to all players. 
The player with rank \(1\) becomes the leader. 
Details of the initialization phase is deferred to Section \ref{sec:SDI-iniPhase}.  


\begin{enumerate}
    \item Initialization phase: estimate the total number of players \(M\) and assign ranks to all players. \begin{itemize}
        \item Player with rank \(1\) becomes the leader. 
    \end{itemize}
    \item Exploration-Exploitation phase: \begin{itemize}
        \item Exploitation: followers exploit empirical optimal arms. 
        \item Parsimonious exploration: the leader parsimoniously explore empirical sub-optimal arms.  
        \item United exploration: all players rally to explore some empirical optimal arms whose capacities have not been well estimated. 
    \end{itemize}
    \item Communication phase: When the leader needs to update his decision, he initializes a round of communication and send them to followers.
\end{enumerate}

\begin{algorithm}[htp]
    \caption{\texttt{DPE-SDI}}
    \label{alg:dpe_sdi}
    \begin{algorithmic}[1]
        \State Initialize parameters: 
        \newline \(i, M\gets 0, \mathcal{L}_t \gets 1, \mathcal{S}_t\gets [K], 
         \bm{m}^{l}_t\gets (1,\ldots,1)^T, 
          \newline  \bm{m}^{u}_t\gets (K,\ldots,K)^T, 
         \hatbm{\mu}_t,\hatbm{\nu}_t\gets (0,\ldots,0)^T\)
        \State \((i,M)\gets\texttt{DPE-SDI.Init}()\)
        \label{algo:SDI-init}     
        \While{\(t\le T\)}                
            \If{\(i=1\)}      
                \State \multiline{\((\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\gets\texttt{DPE-SDI.Explo}(i,M,\mathcal{S}_t, \mathcal{L}_t, \mathcal{E}_t, \bm{m}^l_t, \bm{m}^u_t)\)}
                \State \(\mathcal{S}_{\text{pre}},\bm{m}^l_{\text{pre}},\bm{m}^u_{\text{pre}} \gets \mathcal{S}_t, \bm{m}^l_t, \bm{m}^u_t\)      
                \State \multiline{\((\mathcal{S}_t, \mathcal{L}_t, \mathcal{E}_t, \bm{m}^l_t, \bm{m}^u_t)\gets\texttt{DPE-SDI.Update}(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\)}
                \State \multiline{\(\texttt{DPE-SDI.CommSend}(\mathcal{S}_t, \mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t, \mathcal{S}_{\text{pre}},\bm{m}^l_{\text{pre}},\bm{m}^u_{\text{pre}})\)}
            \ElsIf{\(i\neq 1\)}
                \State \multiline{\(\texttt{DPE-SDI.Explo}(i,M,\mathcal{S}_t, \mathcal{L}_t, \mathcal{E}_t, \bm{m}^l_t, \bm{m}^u_t)\)}
                \State \multiline{\((\mathcal{S}_t, \mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t)\gets\texttt{DPE-SDI.CommRece}(\mathcal{S}_t, \bm{m}^l_t, \bm{m}^u_t)\)}
            \EndIf
        \EndWhile
    \end{algorithmic}
\end{algorithm}

\subsection{Initialization Phase}
\label{sec:SDI-iniPhase}

\begin{algorithm}[htp]
    \caption{\(\texttt{DPE-SDI.Init}()\)}
    \label{alg:dpe_sdi_init}
    \begin{algorithmic}[1]
        \State\algorithmicensure rank \(i\), the number of players \(M\)
        % \State \LeftComment{Initialization Phase}
        \State \(M \gets\text{Rally}\) \label{algline:rally}
        \State \(i\gets \text{Orthogonal}(M)\) \label{algline:rankassignment}
    \end{algorithmic}
\end{algorithm}

The initialization phase in Algorithm~\ref{alg:dpe_sdi_init} contains two parts: probing the total number of players \(M\) (Rally in line~\ref{algline:rally}), and assigning each player a rank from \(\{1,2,\ldots, M\}\) (Orthogonal in line~\ref{algline:rankassignment}). 
This procedure is different from the common one of MMAB: first assign external ranks via orthogonalization, and then assign internal rank and estimate \(M\) via sequential hopping, e.g., in DPE1~\cite{wang_optimal_2020} and SIC-MMAB~\cite{boursier_sic-mmab_2019}. 

Our initialization phase is much simpler than the common one, thanks to the SDI feedback. 
From this feedback, players can easily observe the number of players \(M\) by rallying at the same arm once. 
Knowing \(M\), one just need to orthogonalize \(M\) players to \(M\) arms and the player's orthogonalized arm index can be used as its internal rank directly. 
We employ an orthogonalization approach similar to \cite{wang_optimal_2020}'s to assign \(M\) players to \(M\) different arms. 
We provide the detail of orthogonalization and prove that its expected time slots \(\E[T_0]\) is no greater than \(M^3+M^2\) in Appendix~\ref{appsub:dpe_sa_init}.

% For Rally at the first time slot, all players just choose arm 1 (or any other pre-determined arm). Then from SDI $a_1(1)$, all players would observe the total number of players \(M\). 
% As the number of players \(M\) is known, we can apply a randomized orthogonalization. 
% Each player starts with a rank \(M+1\).
% The algorithm runs in rounds and each round contains \(M+1\) time slots. 
% In the beginning of a round, if the player's rank is \(M+1\), then he uniformly choose an arm \(i\in [M]\) to play,
% and if its rank \(i\) is less than \(M+1\), he plays arm \(i\).
% If player with rank \(M+1\) receives the feedback \(a_{j,t} = 1\), he updates his rank to \(j\);
% otherwise, there are other players sharing the arm and his rank is still \(M+1\). 
% In the round's subsequent \(M\) time slots, each player always chooses their rank's corresponding arm 
% except that at the \((i+1)\)th time slot she chooses arm \(M+1\). 
% If each player was orthogonally assigned with a rank in \(\{1,2,\ldots,M\}\), in these subsequent \(M\) time slots, no sharing (i.e., \(a_{k,t} > 1\)) would happen. Or otherwise, all players will experience arm sharing at least once. 
% \textbf{Appendix.} give the \(\E[T_0]\) analysis. 


\subsection{The Exploration-Exploitation Phase}

The exploration-exploitation phase's detail is illustrated in Algorithm~\ref{alg:dpe_sdi_explo}. 
It consists of exploitation, parsimonious exploration and united exploration. 
Note that exploitation and parsimonious exploration are parallel, 
in which all players exploit empirical optimal arms while the leader sometimes deviates to explore empirical sub-optimal ones.

Denote \(\hatbm{a}^*_t \coloneqq (\hat{a}_{1,t}^*, \ldots, \hat{a}_{K,t}^*)\) as the empirical optimal assignment profile according to observations up to time \(t\). 
Denote the empirical optimal arm set as \(\mathcal{S}_t\coloneqq \{k: \hat{a}_{k,t}^* > 0\}\)
and the empirical least favored arm among empirical optimal arms as \(\mathcal{L}_t\).
We also denote the upper and lower confidence bounds of shareable resources as \(\bm{m}_t^l \coloneqq (m_{1,t}^l,\ldots, m_{K, t}^l)\) and \(\bm{m}_t^u \coloneqq (m_{1,t}^u,\ldots, m_{K, t}^u)\).
Note that the leader does not transmit the empirical optimal action \(\hatbm{a}_{k,t}^*\in \N^K\) to its followers, which might take plenty of steps for communication in one update. 
Because followers can recover \(\hatbm{a}^*_t\) from \(\mathcal{S}_t, \mathcal{L}_t, \bm{m}^l_t\) (at Algorithm~\ref{alg:dpe_sdi_explo}'s Line~\ref{alg:dpe_sdi_recover}): 
the \(\hat{a}_{k,t}^*\) is equal to \(m_{k,t}^l\) for \(k\) in \(\mathcal{S}_t\) but not \(\mathcal{L}_t\)
and, the \(\hat{a}_{\mathcal{L}_t,t}^*\) of the empirical least favored arm is equal to \(M - \sum_{k\in\mathcal{S}_t, k\neq \mathcal{L}_t} m_{k,t}^l\).

\begin{algorithm}[htp]
    \caption{\texttt{DPE-SDI.Explo}\((i,M,\mathcal{S}_t, \mathcal{L}_t, \mathcal{E}_t, \bm{m}^l_t, \bm{m}^u_t)\)}
    \label{alg:dpe_sdi_explo}
    \begin{algorithmic}[1]
        \State \algorithmicensure \((\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\)
        \State \(\hatbm{a}_t^* \gets \text{Recover}(\mathcal{S}_t, \mathcal{L}_t, \bm{m}_t^l)\) \label{alg:dpe_sdi_recover}
        \For{\(M\) times} \Comment{Parsimonious exploration}
            \State \(j\gets \text{Rotate}(i,M,\hatbm{a}_t^*,t)\) \label{alg:dpe_sdi_rotate}
            \If{\(i\neq 1\)}\Comment{Follower}
                \State{Play arm \(j\)} 
            \ElsIf{\(i=1\)}\Comment{Leader}
                \If{\(\mathcal{E}_t \neq \emptyset\) and \(j = L_t\)}
                    \State{w.p. $1/2$, \(k\gets l\sim\mathcal{E}_t\) uniformly}
                    \State{w.p. $1/2$,  \(k\gets j\)}
                \Else 
                    \State{ \(k\gets j\)}
                \EndIf
                \State Play arm \(k\)
                \State \(S^{\text{IE}}_{k,t} \gets S^{\text{IE}}_{k,t}  + \frac{r_{k,t}}{\hat{a}^*_{k,t}}, \tau_{k,t}\gets \tau_{k,t} + 1\)
            \EndIf
            \State \(t\gets t+1\).
        \EndFor

        \State \(\mathcal{S}'_t\gets \{k\in\mathcal{S}_t: m_{k,t}^{l} \neq m_{k,t}^{u}\}.\)
        \For{\(k\in\mathcal{S}'_t\)}
            \State All players choose arm \(k.\) \Comment{United exploration}
            \If{\(i=1\)}
                \State \(S^{\text{UE}}_{k,t} \gets S^{\text{UE}}_{k,t}  + r_{k,t}\)
                \State \(\iota_{k,t} \gets \iota_{k,t} + 1\)
            \EndIf
            \State \(t\gets t+1\)
        \EndFor
    \end{algorithmic}
\end{algorithm}

\textbf{Exploitation.} Players cooperate to exploit arms according to the empirical optimal assignment profile \(\hatbm{a}^*_t\) and they rotate over the empirical optimal arms in different time slots. 
To rotate players over different arms, we take \((i+t)\Mod{M}\) as their circulating rank for choosing arms in time slot \(t\).
Note that in the profile, several players may share the same arm, e.g., when \(\hat{a}^*_{k,t} > 1\) for some \(k\).
To suit this, we apply a rotate rule (Algorithm~\ref{alg:dpe_sdi_explo}'s Line~\ref{alg:dpe_sdi_rotate}):
at time slot \(t\), player with rank \(i\) plays arm \(j\) such that \(\sum_{n=1}^{j} \hat{a}_{n,t}^* \ge (i+t)\Mod{M} > \sum_{n=1}^{j-1} \hat{a}_{n,t}^*\). That means players with circulating rank greater than \(\sum_{n=1}^{j-1} \hat{a}_{n,t}^*\) and no less than \(\sum_{n=1}^{j} \hat{a}_{n,t}^*\) chooses arm \(j\).

\textbf{Individual exploration.} 
We define a type of exploration called individual exploration (IE) when the arm's resources are not over occupied, i.e, \(a_{k,t} \le m_k\).
The simplest case of IE happens when only a single player chooses an arm,
but it also includes cases that several players share an arm.
For example, we note that the leader's actions during exploitation and parsimonious exploration can all be regarded as IEs because \(\hat{a}_{k,t}^* \le m_{k,t}^l\).
Divided by \(a_{k,t}\), IE's rewards can be employed to estimate the reward mean \(\hat{\mu}_{k,t} = {S}_{k,t}^{\text{IE}}/\tau_{k,t}\), where \({S}_{k,t}^{\text{IE}}\) is the summation of IE's reward feedback (divided by the number of players on arm \(k\)) up to time slot \(t\) and \(\tau_{k,t}\) is the number of IE times for arm \(k\) up to time slot \(t\).

\textbf{Parsimonious exploration.} 
Only when the leader plays the empirical least favored arm \(\mathcal{L}_t\) can he, with a  $0.5$ probability, 
explore an empirical sub-optimal arm whose KL-UCB index~\cite{cappe_kullback-leibler_2013} is larger than \(\mathcal{L}_t\)'s. Denote $u_{k,t}$ as the KL-UCB index as 
\(
    u_{k,t} = \sup\{q\ge 0: \tau_{k,t}\kl(\hat{\mu}_{k,t}, q)\le f(t)\},
\)
where $f(t) = \log (t) + 4 \log\log (t)$. 
We denote \(\mathcal{E}_t\) as a subset of empirical sub-optimal arms whose KL-UCB index is larger than arm \(\mathcal{L}_t\)'s, i.e., \(\mathcal{E}_t\coloneqq \{k: u_{k,t} \ge \hat{\mu}_{\mathcal{L}_t,t}, a_{k,t} = 0\}.\)
We note that the parsimonious exploration idea was first made in~\cite{combes_learning_2015} for learning-to-rank algorithms and was further utilized in~\cite{wang_optimal_2020} for multiple player setting. 

\textbf{United exploration.}
UE refers to all \(M\) players rallying on an arm so that they can observe a sample of random variable \(m_kX_k\) when its resources are fully utilized. 
Collecting this kind of observation is crucial in calculating an arm's shareable resources \(m_k\) (see Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update})).
Let arm set \(\mathcal{S}'_t=\{k:a_{k,t} > 0, m_{k,t}^{l} \neq m_{k,t}^{u}\}\) contain empirical optimal arms whose amounts of resources have not been learnt.
In each round of exploration-exploitation phase, all \(M\) players rally to explore each arm of \(\mathcal{S}'_t\) once in turn.
%  in \(\abs{\mathcal{S}'}\) time slots.
Denote \(S_{k,t}^{\text{UE}}\) as the total reward of UE from arm \(k\) up to time \(t\), \(\iota_{k,t}\) as the number of UE times for arm \(k\) up to time \(t\), and the empirical mean estimate of \(\E[m_kX_k]\) is \(\hat{\nu}_{k,t}\coloneqq S_{k,t}^{\text{UE}} / \iota_{k,t}\).

\begin{algorithm}[htp]
    \caption{\texttt{DPE-SDI.Update}\((\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\)}
    \label{alg:dpe_sdi_update_stats}
    \begin{algorithmic}[1]
        % \State \algorithmicrequire \((\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\)
        \State \algorithmicensure \((\mathcal{S}_t, \mathcal{L}_t, \mathcal{E}_t, \bm{m}^l_t, \bm{m}^u_t)\)
        \If{\(i=1\)}
            \State \(\hat{\mu}_{k,t}\gets {S}_{k,t}^{\text{IE}}/ {\tau}_{k,t}, \hat{\nu}_t\gets {S}_{k,t}^{\text{UE}} / {\iota}_{k,t},\,\forall k\)
            \State Updates \(\bm{m}^{l}_t, \bm{m}^{u}_t\) via Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update})
            \State{\(\hatbm{a}^*_t\gets \Oracle(\hat{\bm{\mu}}_t, \bm{m}^l_t)\)}
            \State{\(\mathcal{S}_t\gets \{k: \hat{a}_{k,t}^* > 0\}\)}
            \State{\(\mathcal{L}_t\gets \argmin_k\{\hat{\mu}_{k}:a_{k,t} > 0\}\)}
            \State{$\mathcal{E}_t\gets \{k: u_{k,t} \ge \hat{\mu}_{L_t,t}, a_{k,t} = 0\}.$}
        \EndIf
    \end{algorithmic}
\end{algorithm}


\textbf{Leader updates statistics. }
At the end of exploration and exploitation phase, the leader updates its records as in Algorithm~\ref{alg:dpe_sdi_update_stats}. 
Especially, we update the shareable resources \(m_k\)'s lower and upper confidence bounds as follows:
\begin{align}
    & m_{k,t}^l = \label{eq:lower_bound_update}\\
    &\max\left\{m_{k,t}^l, \ceil{\frac{\hat{\nu}_{k,t}}{\hat{\mu}_{k,t} + \phi(\tau_{k,t}, \delta) + \phi(\iota_{k,t}, \delta)}}\right\},\nonumber\\
    &m_{k,t}^u = \label{eq:upper_bound_update}\\
    & \min\left\{m_{k,t}^u, \floor{\frac{\hat{\nu}_{k,t}}{\hat{\mu}_{k,t} - \phi(\tau_{k,t}, \delta) - \phi(\iota_{k,t}, \delta)}}\right\},\nonumber
\end{align}
where the function
\(
    \phi(x,\delta) \coloneqq \sqrt{\left(1+\frac{1}{x}\right)\frac{\log(2\sqrt{x+1}/\delta)}{2x}}.
\)
Their derivations are provided in Appendix~\ref{app:update_ci}. 


%  $\phi(\tau_{k,t},\delta) + \phi(\iota_{k,t},\delta) < \hat{\mu}_{k,t}$,

% \textbf{Individual exploration.} As a contrast to united exploration (UE), we define another type of exploration called individual exploration (IE) when one assures \(a_{k,t} < m_k\).
% The simplest case of IE happens when an individual player chooses arm \(k\),
% but it also includes cases that several players share an arm.
% For example, we note the leader's actions during parsimonious exploration can all be regarded as IEs.
% So, divided by \(a_{k,t}\), IE's rewards can be employed to estimate the reward mean \(\hat{\mu}_{k,t} = \bm{S}_{k,t}^{\text{IE}}/\tau_{k,t}\), where \(\bm{S}_{k,t}^{\text{IE}}\) is the summation of IE's reward feedback (divided by the number of players on arm \(k\)) up to time slot \(t\) and \(\tau_{k,t}\) is the number of IE times for arm \(k\) up to time slot \(t\).
% We note that the leader's actions during parsimonious exploration can  

% Utilize the capacity estimator and uniform confidence interval;



\subsection{Leader-Follower Communication Protocol}\label{subsec:dpe_sdi_comm}

After each round of the exploration-exploitation phase, the leader updates its information. 
If there are any changes of \(\mathcal{S}_t, \mathcal{L}_t,\bm{m}^{l}_t, \bm{m}^{u}_t\), 
leader will initialize a round of communication to update these information of followers. 
For simplicity, we illustrate the communication as 6 sub-blocks as follows. 
Some potential improvements of the communication are discussed in Appendix~\ref{appsub:dpe_sa_comm}.

\begin{enumerate}
	\item Initial block: the leader signifies followers to start communication. 
	\item Second block: notify a subset of arms to be removed from \(\mathcal{S}_t\), i.e., \(\mathcal{S}_{\text{pre}}\setminus\mathcal{S}_t\).
	\item Third block: notify a subset of arms to be added in \(\mathcal{S}_t\), i.e., \(\mathcal{S}_t\setminus \mathcal{S}_{\text{pre}}\). 
	\item Forth block: notify the empirical least favored arm \(\mathcal{L}_t\) among \(\mathcal{S}_t\).
	\item Fifth phase: update capacities' lower bound \(\hatbm{m}^l_t\).
	\item Sixth phase: update capacities' upper bound \(\hatbm{m}^u_t\).
\end{enumerate}

\begin{algorithm}[htp]
    \caption{\texttt{DPE-SDI.CommSend}\\\((\mathcal{S}_t, \mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t, \mathcal{S}_{\text{pre}},\bm{m}^l_{\text{pre}},\bm{m}^u_{\text{pre}})\)}
    \label{alg:dpe_sdi_update_stats}
    \begin{algorithmic}[1]
        \For{\(M\) times}\Comment{Initial block}
            \State{Play arm \(\hat{k}_t^*\) with highest empirical mean}
        \EndFor
        \For{\(j\in\{2,3,4,5,6\}\)}\Comment{2nd-6th block}
            \For{\(k\in [K]\)}
                \If{\(j\)-th block's condition}
                    \State Play arm \(k\)
                \Else
                    \State Play arm \((k+1)\Mod{M}\)
                \EndIf
            \EndFor
        \EndFor
        % \For{\(k\in [K]\)}\Comment{2nd block}
        %     \If{\(k\in\mathcal{S}_{\text{pre}}\setminus\mathcal{S}_t\)}
        %         \State Play arm \(k\)
        %     \Else
        %         \State Play arm \((k+1)\Mod{M}\)
        %     \EndIf
        % \EndFor
        % \For{\(k\in [K]\)}\Comment{3rd block}
        % \If{\(k\in\mathcal{S}_t\setminus \mathcal{S}_{\text{pre}}\)}
        %     \State Play arm \(k\)
        % \Else
        %     \State Play arm \((k+1)\Mod{M}\)
        % \EndIf
        % \EndFor
        % \For{\(k\in [K]\)}\Comment{4th block}
        % \If{\(k = \mathcal{L}(t)\)}
        %     \State Play arm \(k\)
        % \Else
        %     \State Play arm \((k+1)\Mod{M}\)
        % \EndIf
        % \EndFor
        % \For{\(k\in [K]\)}\Comment{5th block}
        % \If{\(m_{k,t}^l > m_{k,\text{pre}}^l\)}
        %     \State Play arm \(k\)
        % \Else
        %     \State Play arm \((k+1)\Mod{M}\)
        % \EndIf
        % \EndFor
        % \For{\(k\in [K]\)}\Comment{6th block}
        % \If{\(m_{k,t}^u < m_{k,\text{pre}}^u\)}
        %     \State Play arm \(k\)
        % \Else
        %     \State Play arm \((k+1)\Mod{M}\)
        % \EndIf
        % \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[htp]
    \caption{\texttt{DPE-SDI.CommRece}\((\mathcal{S}_t, \bm{m}^l_t, \bm{m}^u_t)\)}
    \label{alg:dpe_sdi_update_stats}
    \begin{algorithmic}[1]
        \If{\(a_{\hat{k}_t^*,t} > \hat{a}^*_{\hat{k}_t^*,t}\)}
            \State Start communication  \Comment{Initial block}
            \State Wait till 2nd block
            \For{\(j\in\{2,3,4,5,6\}\)}\Comment{2nd-6th block}
                \For{\(k\in [K]\)}
                    \State Play arm \(k\)
                    \If{\(a_{k,t} > \hat{a}^*_{k,t}\) and \(k\in\mathcal{S}_t\)}
                        \State \(j\)-th block's update
                    \EndIf
                \EndFor
            \EndFor
            % \For{\(k\in [K]\)}\Comment{2nd block}
            %     \State Play arm \(k\)
            %     \If{\(a_{k,t} > \hat{a}^*_{k,t}\) and \(k\in\mathcal{S}_t\)}
            %         \State Remove arm \(k\) from \(\mathcal{S}_t\)
            %     \EndIf
            % \EndFor
            % \For{\(k\in [K]\)}\Comment{3rd block}
            %     \State Play arm \(k\)
            %     \If{\(a_{k,t} > \hat{a}^*_{k,t}\) and \(k\in\mathcal{S}_t\)}
            %         \State Add arm \(k\) to \(\mathcal{S}_t\)
            %     \EndIf
            % \EndFor
            % \For{\(k\in [K]\)}\Comment{4th block}
            %     \State Play arm \(k\)
            %     \If{\(a_{k,t} > \hat{a}^*_{k,t}\) and \(k\in\mathcal{S}_t\)}
            %         \State \(\mathcal{L}_t \gets k\)
            %     \EndIf
            % \EndFor
            % \For{\(k\in [K]\)}\Comment{5th block}
            %     \State Play arm \(k\)
            %     \If{\(a_{k,t} > \hat{a}^*_{k,t}\) and \(k\in\mathcal{S}_t\)}
            %         \State \(m_{k,t}^l \gets m_{k,t}^l+1\)
            %     \EndIf
            % \EndFor
            % \For{\(k\in [K]\)}\Comment{6th block}
            %     \State Play arm \(k\)
            %     \If{\(a_{k,t} > \hat{a}^*_{k,t}\) and \(k\in\mathcal{S}_t\)}
            %     \State \(m_{k,t}^u \gets m_{k,t}^u - 1\)
            % \EndIf
            % \EndFor
        \EndIf
    \end{algorithmic}
\end{algorithm}

\emph{Initial block:} 
When the leader needs to update followers' information after an exploration-exploitation phase, 
he stops at the arm \(\hat{k}^*_t\) with highest empirical mean.
Followers start the next round's exploration-exploitation phase (i.e., play arms of \(\hatbm{a}^*_t\) in turn). 
In subsequent time slots, followers playing arm \(\hat{k}^*_t\) would observe \(a_{\hat{k}^*_t,t} > m_{\hat{k}^*_t,t}^l\),
which violates the profile \(\hatbm{a}^*_t\),
and realize that a communication starts. 
We note that this ad-hoc communication initialization is crucial for \texttt{DPE-SDI} and when considering weaker SDA feedback, such communication is invalid.

In the remaining 5 blocks, 
followers cooperate to play same arms and rotate over all \(K\) arms once in each block.
% all followers always play the same arm and play all \(K\) arms in turn.
Each block is exactly \(K\) time slots. 
When these followers are on an arm \(k\), the number of players sharing arm \(k\) is at least \(M-1\), i.e., \(a_{k,t} \ge M-1\). 
When the leader wants to update information related to arm \(k\) in some blocks, he will choose arm \(k\) when followers play the arm.
Then all followers observe \(a_{k,t} = M\). 
This is a signal for updating arm \(k\)'s related information.

For these 5 blocks, the \(a_{k,t} = M\) signal respectively stands for 
removing arm \(k\) from empirical optimal arm set \(\mathcal{S}_t\) (2nd),
adding arm \(k\) to \(\mathcal{S}_t\) (3rd),
updating arm \(k\) as the empirical least favored arm \(\mathcal{L}_t\) (4th),
increasing arm \(k\)'s capacity lower bound \(m_{k,t}^l\) by 1 (5th), and 
decreasing arm \(k\)'s capacity upper bound \(m_{k,t}^u\) by 1 (6th).


% \subsection{Regret Analysis}
% \subsubsection{RegA}

==> sections/introduction_backup.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Introduction}

Multi-armed bandits (MAB)~\cite{lai_asymptotically_1985,bubeck_regret_2012} is a canonical sequential decision 
making model for studying the 
\textit{exploration} vs. \textit{exploitation} trade-off.
In stochastic MAB, a player pulls one arm among \(K\in\N_+\) arms per time slot and receives a reward from this pulled arm, 
which is generated by a random variable.
To maximize the total reward, the player needs to
make a balance between choosing the arms with high uncertainty in 
their reward mean (exploration) and 
choosing the empirical good arms (exploitation).  
% the player needs to explore which arm is the optimal but can never find it for sure.
% Another kinds of 
After MAB, \citet*{anantharam_asymptotically_1987} considered the multiple-play multi-armed bandits (MP-MAB) model in which the payer can pull \(M\in\{2,\ldots,K-1\}\) arms from \(K\) arms per time slot. 
% multiple-play multi-armed bandits (MP-MAB).

Recently, the decentralized \emph{multiple players} multi-armed bandits (MMAB) was proposed~\cite{liu_decentralized_2010,anandkumar_distributed_2011}. 
Instead of one player choosing \(M\) arms as in MP-MAB, 
there are \(M\) players in MMAB and each of them pulls one arm from \(K\) arms per time slot \emph{without knowing others' selections.} 
% in the same MAB of \(K\) arms. 
To maximize these \(M\) players' total reward, MMAB also needs to deal with the exploration-exploitation trade-off as the MAB and MP-MAB did. 
One particularity of MMAB is how to define the reward when several players choose the same arm at the same time. 
One typical setting is that all of them get zero reward, i.e., these players have a \emph{collision},
which was first motivated by cognitive radio network~\cite{jouini_multi-armed_2009}.
Another type of setting is that each of them gets an independent reward from the arm, i.e., the non-collision setting,
which was first motivated by distributed system~\cite{landgren_distributed_2016}. 


However, in real world applications, 
neither every channel of cognitive radio network can only support the traffic of a single user nor every edge computer in distributed systems can serve any large number of clients simultaneous.   
More concretely, consider a cognitive radio network consisting of \(K\) channels (arms) and \(M\) secondary users (players). 
Each secondary user chooses one channel to transmit information per time slot repeatedly.
If the selected channel is available at the time slot, the user can successfully transmit his information. 
Although channel competition might occur when many users choose the same channel,
some channels with a wide bandwidth (shareable resources) can fully support the traffic of several users simultaneous. 
To maximize the total transmission throughput, some players might need to \emph{share} a channel which has a wide bandwidth, especially,
when the channel also has a high availability rate. 
Furthermore, in mobile edge computing applications, 
each edge devices (arm) may have multiple computing units (resources), and thus can be shared by multiple users (players).
Similar examples also appear in the distributed system, online advertisement placement, and many other applications. 


%It can be regarded as a trade-off of collision model and non-collision model. 

To capture this wide range of applications,
we propose the multiple player multi-armed bandits with finite shareable resources arms (\texttt{MMAB-SA}) model.   
We introduce the \emph{shareable} arms setting into MMAB as a trade-off between the collision and non-collision formulations.  
This setting allows several players to share an arm (non-collision), but their rewards are not independent and are restricted by the arm's total shareable resources (quasi-collision). 
Formally, each arm is associated with both a ``per-load'' reward random variable \(X_k\) and a finite resources capacity \(m_k\in\N_+\). 
When \(a_k\) players choose arm \(k\), they acquire a reward \(\min\{a_k, m_k\}X_k\). 
It means that if the number of players sharing the arm does not exceed the arm's shareable resource capacity, i.e., \(a_k \le m_k\), then \(a_k\) out of these \(m_k\) resources are utilized; or otherwise, all \(m_k\) resources would be utilized. 
The reward \(X_k\) can model whether a channel is available or not, or the instantaneous computation speed of an edge computer, etc. 
We note that both the reward mean \(\mu_k\coloneqq \E[X_k]\) and the resources \(m_k\) are unknown to players. 


Recently, several sophisticated algorithms for MMAB were proposed, 
e.g., musical chair~\cite{rosenski_multi-player_2016}, MCTopM~\cite{besson_multi-player_2018}, SIC-MMAB~\cite{boursier_sic-mmab_2019}, and DPE1~\cite{wang_optimal_2020}.
% For example, \citet*{rosenski_multi-player_2016} proposed the Musical Chair algorithm which could spread players to different optimal arms in a decentralized manner. 
% \citet*{besson_multi-player_2018} designed the MCTopM algorithm incorporating index policies like UCB. 
% Utilizing collision information, SIC-MMAB~\cite{boursier_sic-mmab_2019} introduced an explicit communication protocol between players.
% DPE1~\cite{wang_optimal_2020} was the first algorithm achieving the optimal regret bound.
% However, our shareable arms model cannot be simply tackled by these algorithms. 
However, none of the above algorithms can address our shareable arms setting. 
The reason is that the unknown resource capacity of each arm  
and the sharing mechanism further complicate the usual collision setting:
% while collision is only utilized for signaling in MMAB, sharing arms takes two 
(1) instead of avoiding collisions for maximizing total reward in MMAB, 
players in our setting \emph{often have to} play the same arm for the sake of reward,
and how many players are appropriate to share an arm depends on the arm's resource \(m_k\);
(2) instead of taking infrequent collisions only as signals in MMAB, players in our setting needs to \emph{extract information} from the frequent occurrences of arm sharing. 
For the first challenge, we propose decentralized algorithms that can explore (learn) arm's maximum resources capacities and exploit (share) good arms while addressing the classic exploration-exploitation trade-off of MMAB at the same time.
For the second challenge, we designed two types of communication phases (and their corresponding algorithms) to extract information from two types of feedback (see Section~\ref{subsec:feedback}): 
the sharing demand information (SDI) in which players can get the number of players sharing his selected arm, i.e., \(a_k\); and the sharing demand awareness (SDA) in which players know whether their selected arms are shared or not \(\1{a_k>1}\).
The latter only requires \(1\)-bit information as feedback, hence it is easier to realize in practice. 
Our contributions are as follows. 
\begin{itemize}
    \item We propose the \texttt{MMAB-SA} model which significantly expands the application scope of MMAB. It allows several players to share an arm with shareable resources. 
    When players share an arm, they not only observe their reward attained from the arm, but also addition feedback about the sharing demand, e.g. the SDI feedback or the SDA feedback. 
    % Especially, we consider the SDI and SDA
    
    \item We design the \texttt{DPE-SDI} and \texttt{SIC-SDA} algorithms to address \texttt{MMAB-SA} under the SDI and SDA feedback respectively.
    With the number of players sharing an arm from the SDI feedback, \texttt{DPE-SDI} has a much simpler initialization phase than the usual one in MMAB. 
    Apart from estimating arm's reward means \(\mu_k\), players also need to estimate arms' resources \(m_k\). 
    This estimation task and the shareable arm setting requires more information exchange between players than MMAB.
    To address the issue, we devised two communication protocol for \texttt{DPE-SDI} and \texttt{SIC-SDA} algorithms respectively.
    We also rigorously prove that both algorithms have logarithmic regrets.  
    
    % \item We designed the \texttt{SIC-SDA} algorithm to handle \texttt{MMAB-SA} under the SDA feedback.
    
    \item We conduct simulations to validate and compare the performance of \texttt{DPE-SDI} and \texttt{SIC-SDA}.
\end{itemize}

\subsection{Other related works}

Our work falls into the research line of (decentralized) multiple player multi-armed bandits (MMAB),
which was first studied by~\cite{liu_decentralized_2010,anandkumar_distributed_2011}.  
One crucial feature in this MMAB model is the collision setting: 
if more than one players choose the same arm, all of them will receive zero reward.
Recently, \citet*{rosenski_multi-player_2016} proposed the Musical Chair algorithm which could spread players to different optimal arms in a decentralized manner. 
\citet*{besson_multi-player_2018} designed the MCTopM algorithm incorporating index policies like UCB. 
Utilizing collision information, SIC-MMAB~\cite{boursier_sic-mmab_2019} introduced an explicit communication protocol between players.
DPE1~\cite{wang_optimal_2020} was the first algorithm achieving the optimal regret bound.
Besides the usual collision setting in MMAB,
the non-collision MMAB model was also studied, e.g., in~\cite{landgren_distributed_2016,martinez-rubio_decentralized_2019}.  

Several variants of the MMAB model were also proposed and studied recently. 
One variant considers a more practical heterogenous reward setting~\cite{kalathil_decentralized_2014,nayyar_regret-optimal_2016}, i.e., players face different reward distributions in playing arms. 
It modeled that distributed users utilizing the same equipment (or arm) may earn different rewards due to their different geographic locations.  
\citet*{bistritz_distributed_2018,bistritz_game_2020} proposed the game of thrones algorithm achieving a near-\(O(\log T)\) regret. 
This was the first algorithm which can coordinate players to follow the optimal assignment in a fully decentralized manner 
under a heterogenous reward setting. 
\citet*{boursier_practical_2020} designed an ETC-style algorithm which attained the \(O(\log T)\) regret. 
Another variant of MMAB models took game theoretical results, i.e., Nash equilibrium, into consideration.  
For example, \citet*{boursier_selsh_2020} considered selfish players who might 
deceive other players and race to occupy the best arms for their own good.
A new MMAB model considered the two-sided markets, i.e., both arms and players had preference for choosing each other, e.g.,~\cite{liu_competing_2020,sankararaman_dominate_2021}. 

% start from Decentralized multiple player multi-armed bandits, the history 

% two motivations, collision~\cite{jouini_multi-armed_2009}, non-collision~\cite{landgren_distributed_2016}. 
% However, in real world, neither one cognitive radio only works for one users nor a distributed system can server any number of clients. 
% In this paper, we trade off between these two settings and propose a new decentralized model called multiple player multi-armed bandits with finite capacity shareable arms (MMAB-SA). 

% give the mechanism of shareable arm

% motivate the two feedback setting at the introduction




==> sections/related_works.tex <==
% !TeX root = ../decentralized_sa.tex


\section{Related works}\label{sec:related_works}

Our work falls into the research line of (decentralized) multi-player multi-armed bandits (MMAB),
which was first studied by~\cite{liu_decentralized_2010,anandkumar_distributed_2011}.  
One crucial feature in this MMAB model is the collision setting: 
if more than one players choose the same arm, all of them will receive zero reward.
Recently, \citet{rosenski_multi-player_2016} proposed the musical chair algorithm which could spread players to different optimal arms in a decentralized manner. 
\citet{besson_multi-player_2018} designed the MCTopM algorithm incorporating index policies like UCB. 
Utilizing collision information, SIC-MMAB~\cite{boursier_sic-mmab_2019} introduced an explicit communication protocol between players.
DPE1~\cite{wang_optimal_2020} was the first algorithm achieving the optimal regret bound.
Besides the usual collision setting in MMAB,
the non-collision MMAB model was also studied in~\cite{landgren_distributed_2016,martinez-rubio_decentralized_2019}.  
However, none of the above algorithm can address our \texttt{MMAB-SA} problem due to two challenges we mentioned in Section~\ref{sec:intro}.

In designing our \texttt{DPE-SDI} and \texttt{SIC-SDA} algorithms, we utilize some algorithmic techniques from MAB literature.
The parsimonious exploration idea of \texttt{DPE-SDI} was first made in~\cite{combes_learning_2015} for learning-to-rank algorithm and was further utilized in~\cite{wang_optimal_2020} for MMAB algorithms.
The successive accept and reject mechanism of \texttt{SIC-SDA} was made in~\cite{bubeck_multiple_2013} for top \(k\) arms identification and was utilized to design MMAB algorithms in~\cite{boursier_sic-mmab_2019}.
We further extend the idea to our \texttt{MMAB-SA} case where accepting and rejecting arms not only depends on arm's reward means, but also theirs shareable resources which are unknown a prior.

Several variants of the MMAB model were also proposed and studied recently. 
One variant considers a more practical heterogenous reward setting~\cite{kalathil_decentralized_2014,nayyar_regret-optimal_2016}, i.e., players face different reward distributions in playing arms. 
It modeled that distributed users utilizing the same equipment (or arm) may earn different rewards due to their different geographic locations.  
\citet{bistritz_distributed_2018,bistritz_game_2020} proposed the game of thrones algorithm achieving a near-\(O(\log T)\) regret. 
This was the first algorithm which can coordinate players to follow the optimal assignment in a fully decentralized manner 
under a heterogenous reward setting. 
\citet{boursier_practical_2020} designed an ETC-style algorithm which attained the \(O(\log T)\) regret. 
Another variant of MMAB models took game theoretical results, i.e., Nash equilibrium, into consideration.  
For example, \citet{boursier_selsh_2020} considered selfish players who might 
deceive other players and race to occupy the best arms for their own good.
A new MMAB model considered the two-sided markets, i.e., both arms and players had preference for choosing each other, e.g.,~\cite{liu_competing_2020,sankararaman_dominate_2021}. 

% start from Decentralized multiple player multi-armed bandits, the history 

% two motivations, collision~\cite{jouini_multi-armed_2009}, non-collision~\cite{landgren_distributed_2016}. 
% However, in real world, neither one cognitive radio only works for one users nor a distributed system can server any number of clients. 
% In this paper, we trade off between these two settings and propose a new decentralized model called multiple player multi-armed bandits with finite capacity shareable arms (MMAB-SA). 

% give the mechanism of shareable arm

% motivate the two feedback setting at the introduction




% \section{Related Works}

% Our work falls into the research line of (decentralized) multiple player multi-armed bandits (MMAB),
% which was first studied by~\cite{liu_decentralized_2010,anandkumar_distributed_2011}.  
% One crucial feature in this MMAB model is the collision setting: 
% if more than one players choose the same arm, all of them will receive zero reward.
% Recently, several variants of the MMAB model were proposed. 
% One variant considers a more practical heterogenous reward setting~\cite{kalathil_decentralized_2014,nayyar_regret-optimal_2016}, i.e., players face different reward distributions in playing arms. 
% It modeled that distributed users utilizing the same equipment (or arm) may earn different rewards due to their different geographic locations.  
% \citet{bistritz_distributed_2018,bistritz_game_2020} proposed the game of thrones algorithm achieving a near-\(O(\log T)\) regret. 
% This was the first algorithm which can coordinate players to follow the optimal assignment in a fully decentralized manner 
% under a heterogenous reward setting. 
% \citet{boursier_practical_2020} designed an ETC-style algorithm which attained the \(O(\log T)\) regret. 
% Another variant of MMAB models took game theoretical results, i.e., Nash equilibrium, into consideration.  
% For example, \citet{boursier_selsh_2020} considered selfish players who might 
% deceive other players and race to occupy the best arms for their own good.
% A new MMAB model considered the two-sided markets, i.e., both arms and players had preference for choosing each other, e.g.,~\cite{liu_competing_2020,sankararaman_dominate_2021}. 
% Besides the usual collision setting in MMAB,
% an non-collision MMAB model was also proposed and studied, e.g.,~\cite{landgren_distributed_2016,martinez-rubio_decentralized_2019}.  
% It meant that players can select the same arms and earn independent rewards without influencing each other, i.e., no collision happens. 
% Our work is the first to introduce the shareable arm setting into MMAB.  
% %It can be regarded as a trade-off of collision model and non-collision model. 
% We do allow several players to sharing an arm (non-collision), but their rewards are not independent and are restricted by its total shareable resources (quasi-collision). 
% This shareable arm setting is motivated by real-world applications 
% and it significantly expands the application scope of MMAB.  

% Recently, several sophisticated algorithms for MMAB were proposed.
% For example, \citet{rosenski_multi-player_2016} proposed the Musical Chair algorithm which could spread players to different optimal arms in a decentralized manner. 
% \citet{besson_multi-player_2018} designed the MCTopM algorithm incorporating index policies like UCB. 
% Utilizing collision information, SIC-MMAB~\cite{boursier_sic-mmab_2019} introduced an explicit communication protocol between players.
% DPE1~\cite{wang_optimal_2020} was the first algorithm achieving the optimal regret bound.
% % However, our shareable arms model cannot be simply tackled by these algorithms. 
% However, none of the above algorithms can address our shareable arms setting. 
% The reason is that the unknown resource capacity of each arm  
% and the sharing mechanism further complicate the usual collision setting:
% % while collision is only utilized for signaling in MMAB, sharing arms takes two 
% (1) instead of avoiding collisions for maximizing total reward in MMAB, 
% players in our setting \emph{often have to} play the same arm for the sake of reward,
% and how many players are appropriate to share an arm depends on the arm's resource capacity;
% (2) instead of taking infrequent collisions only as signals in MMAB, players in our setting needs to \emph{extract information} from the frequent occurrences of arm sharing. 
% For the first challenge, we propose decentralized algorithms that can explore (learn) arm's maximum resources capacities and exploit (share) good arms while addressing the classic exploration-exploitation trade-off of MMAB at the same time.
% For the second challenge, we designed two communication phases (and their corresponding algorithms) to extract information from two types of feedback (see Section~\ref{subsec:feedback}): one of them is stronger than the collision information in MMAB, 
% while the other only requires \(1\)-bit information as feedback, hence it is easier to realize in practical. 
% % and the other is similar to (if not weaker than) it. 
% % consider two kinds of sharing demand feedback


% % (2) rather than only for acquiring reward, 
% % playing the same arm bears another the communication at the same time. 

% % as players communicate via collision, playing the same arm is burden 
% % sharing arm complicates the usual collision setting in MMAB:
% % sharing (collision) 

% % prevents these algorithms' viability, especially their communication approaches, 

% % In addition, 

% % {\color{blue}  
% % State the algorithmic difference!
% % }




==> sections/sic_sa_algo_backup.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Synchronization Involved Communication for Sharing Demand Awareness Feedback}
% Borrow as much description as possible from the previous section and try to make the structure simple and the ``improvement and adaption'' clear. 

In this section, we propose the \texttt{SIC-SDA} algorithm to tackle the more difficult SDA feedback. 
Different from observing the number of players sharing an arm, under this setting each player can only observe whether its playing arm is shared or not. 

One challenge in this weaker feedback model is that players cannot distinguish whether an arm sharing \(\1{a_k(t) > 1}\) is for utilizing more resources of a good arm or for communication.
Not being able to differentiate them made the ad-hoc communication protocol used by \texttt{DPE-SDI} invalid. 
We thus propose the pre-defined grid-based \texttt{SIC-SDA} algorithms.
It consists of several phases: 
\begin{enumerate}
    \item Initialization phase:
    \item Exploration Phase: \begin{itemize}
        \item Individual and united explorations
    \end{itemize}
    \item Communication and Successive Accept and Reject: \begin{itemize}
        \item Followers send their observations forth to leader.
        \item Leader update statistics and apply the successive accept and reject procedure.
        \item Leader send his updated information back to followers.  
    \end{itemize}
    \item Exploitation Phase:
\end{enumerate}

% In the initialization phase, all players estimate the number of players \(M\) in the system and 
% each player is assigned with a rank from \(\{1,2,\ldots,M\}\).

% After initialization, the main structure of the \texttt{SIC-SDA} algorithm is 
% to individually and unitedly explore all candidate arms for estimating their reward means and shareable resources,
% and after a phase of explorations, followers communicate their observations to a leader,
% and the leader decides which arms to accept and which to reject and then send these information to followers. 
% Some followers will turn to exploit accepted arms, while others will continue to explore active arms until all players are in exploitation phase.
% (arms that have not been accepted or rejected).

Different from the \texttt{DPE-SDI}'s communication procedure, the leader in \texttt{SIC-SDA} not only utilizes his own observations, but also uses (and receives) other followers' observations.
Because in \texttt{SIC-SDA} followers also participate in exploring sub-optimal arms.
So there are two part of communications in \texttt{SIC-SDA} as we stated above. 


After each phase of exploration, some arms may be rejected as sub-optimal ones, while some may be accepted to be optimal arms and be exploited by some players. 
We call the remaining arms as \textbf{active arms}.
Denote \(\mathcal{K}(t)\) as the set of active arms at time slot \(t\) and \(K(t)\) as the number of active arms at time \(t\). 
Apart from players are exploiting arm, the remaining players are called \textbf{active players}. 
Denote \(M(t)\) as the number of active players at time slot \(t\).
% Followers maintain \(\{\mathcal{K}(t), \bm{m}^l(t), \bm{m}^u(t)\}\), where \(\mathcal{K}(t)\) stands for the set of \textbf{active arms} which have not been rejected or accepted and \(\bm{m}^l(t), \bm{m}^u(t)\) denote the lower and upper confidence bounds of shareable resources.


We note that the successive accept and reject was made in~\cite{bubeck_multiple_2013} for top \(k\) arms identification and was utilized to design MMAB algorithms in~\cite{boursier_sic-mmab_2019}.
We further extend the idea to our MMAB-SA case where accepting and rejecting arms no only depends on \(K(t)\)
and \(M(t)\), but also each arm's among of shareable resources which are unknown a prior.

\begin{algorithm}[htp]
    \caption{\texttt{SIC-SDA}}
    \label{alg:SIC-SDA}
    \begin{algorithmic}[1]
        \State \LeftComment{Initialization Phase:}
        \State Initialize \(\text{ExploitArm} \gets -1\); \(p\gets 1\); \(M(t) \gets M\); \(\mathcal{K}(t)\gets [K]\); \(\bm{S}^{\text{IE}},\bm{S}^{\text{UE}}\gets \bm{0}, \bm{b}\gets \bm{1}\)
        \State \(k \gets \text{Orthogonal}(K)\). 
        \State \((M,i)\gets \text{EstimateM}(k)\). 
        \While{\(\text{ExploitArm} = -1\)}
            \State \LeftComment{Exploration Phase: Individual and United Exploration}
            \State \LeftComment{Leader Update Statistics:} 
            \If{\(i=1\)}
                \State Update \(\bm{m}^l(t), \bm{m}^u(t)\) according to Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update}).
                \State \multiline{Update \(\mathcal{A}(t)\), \(\mathcal{R}(t)\), \(\mathcal{L}(t)\) by Eq.(\ref{eq:accept_set})(\ref{eq:reject_set})(\ref{eq:marginal_arm}).}
            \EndIf

            \State \multiline{\LeftComment{Communication: leader sends \(\mathcal{A}(t)\), \(\mathcal{R}(t)\), \(\mathcal{L}(t), \bm{m}^l(t), \bm{m}^u(t)\) to followers.}}

            \State \LeftComment{Update Statistics:} 
            \State \(M(t) \gets M(t) - \sum_{k\in\mathcal{A}(t)}m_k^l(t)\)
            \State \(\mathcal{K}(t) \gets \mathcal{K}(t)\setminus (\mathcal{A}(t) \cup \mathcal{R}(t) \cup \{\mathcal{L}(t)\}\)

            \If{\(\mathcal{L}(t) \neq \emptyset\)}
                \State  \(\text{ExploitArm}\gets \mathcal{L}(t).\)
            \ElsIf{\(i > M(t)\)}
                \State \multiline{\(\text{ExploitArm}\gets j\)-th accept arm where such that \(\sum_{n=1}^j m_{\sigma'(n)}^l \ge i-M(t) > \sum_{n=1}^{j-1} m_{\sigma'(n)}^l\) where \(\sigma'(n)\) is the \(n\)-th accept arm.}
            \Else 
                \State \LeftComment{Update allocation vector \(\bm{b}\):} Algorithm~\ref{alg:sic-sdi-b}
            \EndIf
            \State \(p\gets p + 1\)  
            
        \EndWhile
    
        \State \LeftComment{Exploitation Phase:} Play the \(\text{ExploitArm}\).
        
    \end{algorithmic}
\end{algorithm}

\subsection{Initialization phase}

We apply the same initialization phase as DPE1~\cite{wang_optimal_2020}, whose objectives are to estimate the number of players \(M\) and to assign a rank for each player.
It consists of two sub-phases: (1) orthogonalizing players to \(K\) arms and denoting the settled arm index as its external rank; (2) assigning the internal ranks to all players according to the times of sharing awareness when these players sequentially hopping among arms. The detailed procedure is described in Appendix~\ref{appsub:sic_sa_init}.


% In initialization phase consists of two phases: orthogonalization and rank assignment. 
% The procedure is the same as~\cite{wang_optimal_2020}'s. We s

\subsection{Exploration Phase}

The exploration phase consists of two parts: individual exploration (IE) and united exploration (UE). 
While the UE part is very similar to DPE-SA's, this IE part is different.
This is because (1) the active arms in \(\mathcal{K}(t)\) of \texttt{SIC-SDA} is explored by \(M(t)\) active players, while the empirical optimal arm set \(\mathcal{S}(t)\) of \texttt{DPE-SDI} is explored by all \(M\) players; (2) \texttt{SIC-SDA} does not employ parsimonious exploration and all players participate the exploration.
Since the number of active arms \(K(t)\) and the number of active players \(M(t)\) change as the algorithm runs, 
when individually exploring arm \(k\), the number of players \(a_k(t)\) may also change. 
However, the \(a_k(t)\) is unobservable under the weaker SDA feedback. 
To infer \(a_k(t)\) in IE, players follow a rule: if a player's rank \(i\) is less then the number of active arms \(K(t)\), he plays arm \(i\); otherwise, he choose the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n)}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n)}^l - 1)\) where \(\sigma(n)\) denotes the \(n\)-active arm among \(\mathcal{K}(t)\). 
To update and record the number of players on each arm in IE,
we introduce an allocation vector \(\bm{b}\in\N^K\). 

\begin{algorithm}
    \caption{Update allocation vector \(\bm{b}\)}\label{alg:sic-sdi-b}
    \begin{algorithmic}
        \State \(\bm{b}\gets \bm{1}.\)
        \If{\(M(t) > \abs{\mathcal{K}(t)}\)}
            \State \(d\gets M(t) - \abs{\mathcal{K}(t)}.\)
            \ForAll{\(k \in \mathcal{K}(t)\)}
            \While{\(d>0\) and \(b_k < m_k^l\)}
                \State \(b_k \gets b_k + 1\); \(d\gets d - 1\).
            \EndWhile
            \EndFor
        \EndIf
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}
    \caption{Individual and United Exploration}
    \begin{algorithmic}
        \State \(\pi \gets i\)
        \For{\(\min{K(t), M(t)}2^p\) times} \Comment{Individual Exploration}
            \If{\(i \le \abs{\mathcal{K}(t)}\)}
                \State Play the \(\pi\)-th active arm.
                \State \(S^{\text{IE}}_{\pi}(t)\gets S^{\text{IE}}_{\pi}(t) + \frac{r_\pi(t)}{b_k}\); \(\pi\gets \pi + 1\).
            \ElsIf{\(i > \abs{\mathcal{K}(t)}\)}
                \State\multiline{Play the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n)}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n)}^l - 1)\) where \(\sigma(n)\) denotes the \(n\)-th active arm.}
            \EndIf
        \EndFor
        \State \(\mathcal{K}'(t) \gets \{k\in\mathcal{K}(t): m_k^l \neq m_k^u\}\)
        \For{\(2^p\) times} \Comment{United Exploration}
            \ForAll{ arm \(k \in \mathcal{K}'(t)\)} 
                \State Play arm \(k\)
                \State \(S^{\text{UE}}_{k}(t)\gets S^{\text{UE}}_{k}(t) + r_k(t)\)
            \EndFor
        \EndFor
        \State \(\hat{\mu}_k(t)\gets {S}_k^{\text{IE}}(t) / {\tau}_k(t), \hat{\nu}(t)\gets {S}_k^{\text{UE}}(t) / {\iota}_k(t),\,\forall k\)
    \end{algorithmic}
\end{algorithm}


\subsection{Communication}
There are two kinds of communications: (1) followers send their IE accumulative reward \(\bm{S}^{\text{IE}(t)}\) to leader, (2) leader sends his updated information \(\mathcal{A}(t)\), \(\mathcal{R}(t)\), \(\mathcal{L}(t), \bm{m}^l(t), \bm{m}^u(t)\) to followers. 

\emph{Followers send \(\bm{S}^{\text{IE}}\) to the leader.}
This communication utilizes the \(\1{a_k(t) \ge 1}\) indicator feedback to transmit information.
In the \(n\)-th phase, each arm is individually explored \(2^n\) times. 
So, a follower's accumulated reward of arm \(k\) till the end of phase \(p\) is at most \(2^{p+1} - 1\) and thus can be transmitted from the follower to leader in \(p+1\) time slots via the \(\1{a_k(t) \ge 1}\) indicator, i.e., one time slot for one bit. 
Especially, we use arm \(1\) as the communication arm.
The leader always play arm \(1\). 
When needing to send bit \(1\) to the leader, the follower plays the arm \(1\). 
This part of communication is mesh-grid: for time slots corresponding to \((j,k)\in [2, \min\{M(t), K(t)\}]\times [K(t)]\), follower with rank \(i = j\) will send arm \(k\)'s IE reward summation \(S^{\text{IE}}_k\) to leader. 

\begin{algorithm}
    \caption{Follower to Leader}
    \begin{algorithmic}
        \For{\((j,k)\in [2, \min\{M(t), K(t)\}]\times [K(t)]\)}
            \If{\(i=1\)}
                \State \multiline{Leader receives \(S^{\text{IE}}_k\) from follower with rank \(j\) in \(p\) time slots.}
            \Else 
                \State \multiline{The follower with rank \(j\) sends \(S^{\text{IE}}_k\) to leader in \(p\) time slots.}
            \EndIf 
        \EndFor
    \end{algorithmic}
\end{algorithm}

\emph{Leader send \(\mathcal{A}(t)\), \(\mathcal{R}(t)\), \(\mathcal{L}(t), \bm{m}^l(t), \bm{m}^u(t)\) to followers. }
This part of communication is similar to \texttt{DPE-SDI}'s \(6\)-block procedure. 
As \texttt{SIC-SDA}'s communication is phase-based, there is no need of an initial block. 
Each block update one of \(\mathcal{A}(t)\), \(\mathcal{R}(t)\), \(\mathcal{L}(t), \bm{m}^l(t), \bm{m}^u(t)\) in \(K(t)\) time slots.
The detail protocol is provided in Appendix~\ref{appsub:sic_sa_comm}




\subsection{Successive Accept and Reject}

Denote \(g(k,j)\) as a special indicator function for distinguishing good arm \(k\) from bad arm \(j\) as follows
\[g(k,j)\coloneqq \1{\hat{\mu}_k(t)- 3\sqrt{\frac{\log (T)}{2\tau_k(t)}} \ge \hat{\mu}_k(t) + 3\sqrt{\frac{\log (T)}{2\tau_k(t)}}},\] 
where $g(k,j) =1$ means that arm \(k\)'s reward mean is higher than arm \(j\)'s with high confidence.
% For an arm \(k\), denote \(\mathcal{B}_k(t) \coloneqq \{i\in\mathcal{K}(t): g(k,i)=0\}\) as  

Accept arm \(k\) if the summation of resources' upper confidence bounds of arms that arm \(k\) is not higher than with high confidence (i.e., \(g(k,j) = 0\)) is no greater than \(M(t)\), i.e.,
\(
    \sum_{j\in\mathcal{K}(t): g(k,j) = 0} m_j^u \le M(t).
\) and the arm's among of resources is well estimated, i.e., \(k\in\mathcal{K}(t)\setminus \mathcal{K}'(t)\).
So, the accept arm set \(\mathcal{A}(t)\) is 
\begin{equation}\label{eq:accept_set}
    \mathcal{A}(t) \gets \left\{k\in\mathcal{K}(t)\setminus \mathcal{K}'(t):  \!\!\!\!\!\!\!\!  \sum_{i\in\mathcal{K}(t): g(k,i) = 0} \!\!\!\!\!\!\!\!  m_i^u \le M(t)\right\}. 
\end{equation}
Reject arm \(k\) if the summation of resources' lower confidence bounds of arms whose reward mean is higher than arm \(k\)'s with high confidence is no less than \(M(t)\), i.e.,
\(
    \sum_{i\in\mathcal{K}(t): g(i,k) = 1} m_i^l \ge M(t).
\) and the arm's among of resources is well estimated.
So, the reject arm set \(\mathcal{R}(t)\) is 
\begin{equation}\label{eq:reject_set}
    \mathcal{R}(t) \gets \left\{k\in\mathcal{K}(t)\setminus \mathcal{K}'(t): \!\!\!\!\!\!\!\! \sum_{i\in\mathcal{K}(t): g(i,k) = 1} \!\!\!\!\!\!\!\! m_i^l \ge M(t)\right\}. 
\end{equation}
An arm \(k\) is the least favored among optimal arms if its reward mean is higher than all other arms with high confidence and its resources' lower confidence bound can cover all active arms, i.e.,
% \(
%     \sum_{i\in\mathcal{K}(t)} g(k,i) = \abs{\mathcal{K}(t)} - 1 \text{ and } m_k^l \ge M(t).
% \)
% The marginal accept arm \(\mathcal{L}(t)\) corresponds to the worst arm among optimal arms and the ``marginal'' means the arms' capacity may only be marginally utilized.   
\begin{equation}\label{eq:marginal_arm}
    \mathcal{L}(t) \gets \left\{\!\! k\in\mathcal{K}(t): \!\!\!  \sum_{i\in\mathcal{K}(t)} \!\!\! g(k,i)\! = \! K(t)\! -\! 1, m_k^l \!\ge\! M(t)\!\!\right\}.
\end{equation}


\subsection{{Synchronization Involved Communication for \emph{Sharing Information} Feedback}}

Becasue the SDI's \(a_k(t)\) feedback directly implies the SDA's \(\1{a_k(t) > 1}\) feedback. 
The \texttt{SIC-SDA} algorithm also works under the stronger SDI feedback. 
We name the adapted algorithm as \texttt{SIC-SDI}.

==> sections/sic_sda_algo.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Synchronization Involved Communication for the SDA Feedback}
% Borrow as much description as possible from the previous section and try to make the structure simple and the ``improvement and adaption'' clear. 

%In this section, we propose the \texttt{SIC-SDA} algorithm to tackle the more difficult SDA feedback. 

We first present the high-level idea of 
the \texttt{SIC-SDA} algorithm, 
which addresses the weaker SDA setting,
% The algorithm is organized into several phases.
We then present the algorithm's phases individually.
% individually.    
Lastly, we provide a logarithmic regret bound for the \texttt{SIC-SDA} algorithm.

% Since the SDI feedback directly implies the SDA's \(\1{a_{k,t} > 1}\) feedback,
% the \texttt{SIC-SDA} algorithm also works under the stronger SDI feedback. 
% We name the adapted one as \texttt{SIC-SDI} for future reference.  
% Finally, we prove that \texttt{SIC-SDA} algorithm has 
% a sub-linear regret of order $\log(T)$. 


\subsection{Overview of the design}

% Different from observing the number of players sharing an arm in SDI, u
% Under the SDA feedback, each player can only observe whether its playing arm is shared or not.
% from which one challenge is derived. 
Recall that in \texttt{DPE-SDI}, leader signals followers by deviating the empirical optimal assignment \(\hatbm{a}_t^*\), e.g., \(a_{k,t} > \hat{a}_{k,t}^*\) while exploiting arms by following \(\hatbm{a}_t^*\), e.g., \(a_{k,t} = \hat{a}_{k,t}^*\). 
However, when \(\hat{a}_{k,t}^*\!>\!1\), both cases imply same feedback \(\1{a_{k,t} \!>\! 1}\!=\! 1\) in the SDA setting. 
% One challenge in this weaker feedback model is that 
% players cannot distinguish whether sharing an arm \(\1{a_{k,t} > 1}\) is for utilizing more resources of a good arm or for communication.
Not being able to differentiate these two cases makes the communication protocol (initial step) used by \texttt{DPE-SDI} not applicable to the SDA feedback. 
% We thus propose the pre-defined grid-based \texttt{SIC-SDA} algorithms.
To address this issue, we propose the \texttt{SIC-SDA} algorithm with phase-based communication protocol.

Algorithm \ref{alg:sic_sda} outlines 
the \texttt{SIC-SDA} algorithm consisting of four phases: \emph{initialization phase,} \emph{exploration phase,}
\emph{communication phase,} and 
\emph{exploitation phase.}   
The objective of \emph{initialization phase} 
is to estimate the number of players \(M\) and to assign a rank to each player,
which is similar to~\cite{wang_optimal_2020}.
% It consists of two sub-phases: (1) orthogonalizing players to \(K\) arms and denoting the settled arm index as its external rank; (2) assigning the internal ranks to all players according to the times of sharing awareness when these players sequentially hopping among arms. 
We present its detailed procedure in Appendix~\ref{appsub:sic_sda_init}.  
After the \emph{initialization phase}, \texttt{SIC-SDA} runs the \emph{exploration phase} and \emph{communication phase} 
iteratively (i.e., in a loop).
In the loop, whenever an optimal arm is identified with high confidence, 
% it has a high confidence in finding an optimal arm,
\texttt{SIC-SDA} will assign players to exploit the arm's resources.
In other words, these players leave the loop and execute \emph{exploitation phase} so to zoom in on the optimal arm.
As the algorithm runs, players in the two-phase loop will gradually enter the \emph{exploitation phase}. 
% We note that \texttt{SIC-SDA} only employs a leader-follower structure in communication phase 
% and all players participate in other phases equally.

% In other words, the leader's action has no different from follower in other phases. 
% It consists of several phases: 
% \begin{enumerate}
%     \item Initialization Phase: learn \(M\) and assign ranks. 
%     \item Exploration Phase: Individual and united explorations.
%     \item Communication and Successive Accept and Reject: \begin{itemize}
%         \item Followers send their observations forth to leader.
%         \item Leader update statistics and apply the successive accept and reject procedure.
%         \item Leader send his updated information back to followers.  
%     \end{itemize}
%     \item Exploitation Phase: player plays its assigned arms to the end. 
% \end{enumerate}

% In the initialization phase, all players estimate the number of players \(M\) in the system and 
% each player is assigned with a rank from \(\{1,2,\ldots,M\}\).

% After initialization, the main structure of the \texttt{SIC-SDA} algorithm is 
% to individually and unitedly explore all candidate arms for estimating their reward means and shareable resources,
% and after a phase of explorations, followers communicate their observations to a leader,
% and the leader decides which arms to accept and which to reject and then send these information to followers. 
% Some followers will turn to exploit accepted arms, while others will continue to explore active arms until all players are in exploitation phase.
% (arms that have not been accepted or rejected).

% Different from the \texttt{DPE-SDI}'s, the leader in \texttt{SIC-SDA} not only utilizes his own observations, but also uses (and receives) other followers' observations.
% Because in \texttt{SIC-SDA} followers also participate in exploring sub-optimal arms.
% So there are two part of communications in \texttt{SIC-SDA}: (1) leader collects follower's observations and (2) leader sends its updated information to followers.  

\begin{algorithm}[htp]
    \caption{\texttt{SIC-SDA}}
    \label{alg:sic_sda}
    \begin{algorithmic}[1]
        \State Initialization: \(\exparm \gets -1\); \(p\gets 1\); \(M_t \gets M\); \(\mathcal{K}_t\gets [K]\); \(\bm{S}^{\text{IE}}_t,\bm{S}_t^{\text{UE}}\gets \bm{0}, \bm{b}_t\gets \bm{1}\)
        \Statex \LeftComment{Initialization phase}
        \State \((i,M)\gets\texttt{SIC-SDA.Init()}\)
        \While{\(\exparm = -1\)}
            \Statex \LeftComment{Exploration phase}
            \State \multiline{\((\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\) 
            \newline\(\gets \texttt{SIC-SDA.Explore}(i, p,\bm{b}_t,\mathcal{K}_t, K_t, M_t)\)}
            \Statex \LeftComment{Communication phase}
            \If{\(i=1\)}\Comment{\textit{Leader}}
                \State \multiline{\((\bm{S}^{\text{IE}}_t,\bm{\tau}_t)\gets\texttt{SIC-SDA.CommBack}()\)}
                \State \multiline{\((\mathcal{A}_t, \mathcal{R}_t, \bm{m}_t^l, \bm{m}_t^u)\) 
                \newline\(\gets\texttt{SIC-SDA.AccRej}(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t, \mathcal{K}_t, M_t)\)\label{alg:sic_sda:line:accrej}} 
                \State \(\texttt{SIC-SDA.CommForth}(\mathcal{A}_t, \mathcal{R}_t,\bm{m}_t^l, \bm{m}_t^u)\)
            \ElsIf{\(i\neq 1\)}\Comment{\textit{Follower}}
               \State \(\texttt{SIC-SDA.CommBack}(i, p, \bm{S}^{\text{IE}}_t)\)
               \State \multiline{\((\mathcal{A}_t, \!\mathcal{R}_t,\!\bm{m}_t^l, \!\bm{m}_t^u)\!\gets\!\texttt{SIC-SDA}\!\texttt{.}\!\texttt{CommForth}()\) }
            \EndIf
            
            \State \multiline{\((\exparm, \mathcal{K}_t, M_t, p)\) 
            \newline\(\gets\texttt{SIC-SDA.Update}(i, p, \mathcal{K}_t, M_t, \mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t)\)}
        \EndWhile
        \Statex \LeftComment{Exploitation phase}
        \State Play the \(\exparm\) to the end.
    \end{algorithmic}
\end{algorithm} 


\noindent
\textbf{Successive accept and reject.} After the exploration and communication phase, some arms may be rejected as sub-optimal arms, 
while some may be accepted as optimal arms.
%  and be exploited by some players. 
While these rejected arms will not be selected and these accepted arms will be exploited,
%  by some players, 
the remaining arms, called \emph{active arms}, will be further explored.
The process of updating active arms is called \emph{successive accept and reject}, which corresponds to \texttt{SIC-SDA.AccRej} (line~\ref{alg:sic_sda:line:accrej}). 
We present its details in Appendix~\ref{appsub:sic_sda_sar}.
Denote \(\mathcal{K}_t\) as the set of active arms at time slot \(t\) and \(K_t=\abs{\mathcal{K}_t}\) as the number of active arms. 
Apart from players exploiting accepted arms, the remaining players,
called \emph{active players},
continue to explore active arms.
%  and are called \emph{active players}.
We denote \(M_t\) as the number of active players at time slot \(t\).
% Followers maintain \(\{\mathcal{K}_t, \bm{m}^l_t, \bm{m}^u_t\}\), where \(\mathcal{K}_t\) stands for the set of \textbf{active arms} which have not been rejected or accepted and \(\bm{m}^l_t, \bm{m}^u_t\) denote the lower and upper confidence bounds of shareable resources.

%\subsection{Initialization phase}

%We apply the same initialization phase as DPE1~\cite{wang_optimal_2020}, whose objectives are to estimate the number of players \(M\) and to assign a rank for each player.
%It consists of two sub-phases: (1) orthogonalizing players to \(K\) arms and denoting the settled arm index as its external rank; (2) assigning the internal ranks to all players according to the times of sharing awareness when these players sequentially hopping among arms. The detailed procedure is described in Appendix~\ref{appsub:sic_sda_init}.


% In initialization phase consists of two phases: orthogonalization and rank assignment. 
% The procedure is the same as~\cite{wang_optimal_2020}'s. We s

\subsection{Exploration Phase}

The exploration phase consists of IE and UE. 
While the UE part is similar to \texttt{DPE-SDI}'s, the IE part is different.
% This is because (1) the active arms in \(\mathcal{K}_t\) of \texttt{SIC-SDA} is explored by \(M_t\) active players, while the empirical optimal arm set \(\mathcal{S}_t\) of \texttt{DPE-SDI} is explored by all \(M\) players; (2) \texttt{SIC-SDA} does not employ parsimonious exploration and all players participate the exploration.
% Since the number of active arms \(K_t\) and the number of active players \(M_t\) change as the algorithm runs, 
In IE, when the number of active players \(M_t\) is greater than the number of active arms \(K_t\), some players need to share arms, i.e., \(a_{k,t}>1\). 
Recall that updating \(\bm{S}_t^{\text{IE}}\) needs to know \(a_{k,t}\), the number of players sharing arms.
However, \(a_{k,t}\) is unobservable under the SDA feedback.
%  which is needed in updating \(\bm{S}_t^{\text{IE}}\).
%  in line~\ref{alg:line:update_ie} of Algorithm~\ref{alg:sic_sda_explore}. 
To infer \(a_{k,t}\) in IE, we design the following arm selection rule.
If a player's rank \(i\) is no greater then \(K_t\), he plays the \(((i+t)\Mod{K_t})\)-th active arm; otherwise, he chooses the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n)}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n)}^l - 1)\), where \(\sigma(n)\) denotes the \(n\)-th active arm among \(\mathcal{K}_t\). 
The inequality maps the rank \(i\) higher than \(K_t\) to the \(j\)-th active arm in \(\mathcal{K}_t\) such that 
the \(a_{k,t}\) does not exceed the arm's shareable resources capacity.
% To update and record the number of players on each arm in IE,
% Vector \(\bm{b}_t\in\N^K\) records how each active arm is shared in IE under the above rule. 
The phase's details are deferred to Appendix~\ref{appsub:sid_sda_explore}.
% This is illustrated in Algorithm~\ref{alg:sic_sda_explore}'s line~\ref{alg:sic_sda_explore:individual_explore_start}-\ref{alg:sic_sda_explore:individual_explore_end} and Algorithm~\ref{alg:sic_sda_update}'s line~\ref{alg:sic_sda_update:b_start}-\ref{alg:sic_sda_update:b_end}.
% \vspace{-10pt}
% \begin{algorithm}[htb]
%     \caption{\(\texttt{SIC-SDA.Explore}(i, p,\bm{b}_t,\mathcal{K}_t, K_t, M_t)\)}
%     \label{alg:sic_sda_explore}
%     \begin{algorithmic}[1]
%         \State \algorithmicensure \(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t\)
%         \For{\(K_t2^p\) times} \Comment{Individual Exploration}\label{alg:sic_sda_explore:individual_explore_start}
%             \If{\(i \le K_t\)}
%                 \State \(j\gets (i+t)\Mod{K_t}\)
%                 \State Play the \(j\)-th active arm.
%                 \State \(S^{\text{IE}}_{j,t}\gets S^{\text{IE}}_{j,t} + {r_{j,t}}/{b_{k,t}}\); \(\tau_{j,t}\gets \tau_{j,t}+1\) \label{alg:line:update_ie}
%             \ElsIf{\(i > K_t\)}
%                 \State\multiline{Play the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n),t}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n),t}^l - 1)\) where \(\sigma(n)\) denotes the \(n\)-th active arm.}
%             \EndIf
%         \EndFor\label{alg:sic_sda_explore:individual_explore_end}
%         \State \(\mathcal{K}'_t \gets \{k\in\mathcal{K}_t: m_{k,t}^l \neq m_{k,t}^u\}\)
%         \For{\(2^p\) times} \Comment{United Exploration}
%             \ForAll{ arm \(k \in \mathcal{K}'_t\)} 
%                 \State Play arm \(k\)
%                 \State \(S^{\text{UE}}_{k,t}\gets S^{\text{UE}}_{k,t} + r_{k,t}\); \(\iota_{k,t}\gets \iota_{k,t}+1\)
%             \EndFor
%         \EndFor
%     \end{algorithmic}
% \end{algorithm}
% % \vspace{-10pt}

\subsection{Communication phase}
% There are two kinds of communications in \texttt{SIC-SDA}: 
\texttt{SIC-SDA}'s communication phase consists of two parts: (1) followers send their IE accumulative reward \(\bm{S}^{\text{IE}}_t\) back to the leader, (2) leader sends his updated information \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t\) to followers. 
Their detailed algorithms are presented in Appendix~\ref{appsub:sic_sda_comm}.

\noindent
\textbf{\texttt{SIC-SDA.CommBack}:} \emph{Followers send \(\bm{S}^{\text{IE}}_t\) to the leader.}
This part utilizes the \(\1{a_{k,t} \ge 1}\) feedback to transmit bit information.
% In the \(n\)-th phase, each arm is individually explored \(2^n\) times. 
% So, a follower's accumulated reward of any arm till the end of phase \(p\) is at most \(2^{p+1} - 1\), and thus can be transmitted from the follower to leader in \(p+1\) time slots via the \(\1{a_{k,t} \ge 1}\) indicator, i.e., one time slot transmits one bit. 
In particular, leader always play arm \(1\).
%  and use it as the communication arm.
% The leader always play arm \(1\). 
% When needing to send bit \(1\) to the leader, 
The follower sends bit \(1\) to leader by playing arm \(1\), which generates an arm sharing indication, and sends bit \(0\) by avoiding arm \(1\).
% The communication has a mesh-grid structure: for time slots corresponding to \((j,k)\in [2, \min\{M_t, K_t\}]\times [K_t]\), follower with rank \(i = j\) will send arm \(k\)'s IE reward summation \(S^{\text{IE}}_k\) to leader. 
% We illustrate this in Appendix~\ref{appsub:sic_sda_comm}.

\noindent
\textbf{\texttt{SIC-SDA.CommForth}:} \emph{Leader sends \(\mathcal{A}_t,\mathcal{R}_t,\mathcal{L}_t,\bm{m}^l_t,\) \( \bm{m}^u_t\) to followers. }
This part is similar to \texttt{DPE-SDI}'s six-step communication. 
As \texttt{SIC-SDA}'s communication is phase-based, it does not need the initial block. 
Each step updates one of \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t\) in \(K_t\) time slots.
% The detail protocol is provided in Appendix~\ref{appsub:sic_sda_comm}.

\noindent
\textbf{\texttt{SIC-SDA.Update}:} After the leader updating followers' information, \texttt{SIC-SDA} will update active players, active arms, and other statistics. We present the details in Appendix~\ref{appsub:sic_sda_update}. 
% \begin{algorithm}
%     \caption{\(\texttt{SIC-SDA.CommBack}(i, p, \bm{S}^{\text{IE}}_t)\)}
%     \label{alg:sic_sda_commback}
%     \begin{algorithmic}
%         \For{\((j,k)\in [2, \min\{M_t, K_t\}]\times [K_t]\)}
%             \If{\(i=1\)}
%                 \State \multiline{Leader receives \(S^{\text{IE}}_{k,t}(j)\) from follower\footnote{We use the \((j)\) of \(S^{\text{IE}}_{k,t}(j)\) to indicate the its player with rank \(j\)'s observation when needed.} with rank \(j\) in \(p+1\) time slots.}
%                 \State \(S_{k,t}^{\text{IE}}(1) \gets S_{k,t}^{\text{IE}}(1) + S^{\text{IE}}_{k,t}(j)\)
%                 \State \(\tau_{k,t} \gets \tau_{k,t} + 2^p\)
%             \ElsIf{\(i=j\)}
%                 \State \multiline{The follower with rank \(j\) sends \(S^{\text{IE}}_{k,t}(j)\) to leader in \(p+1\) time slots.}
%             \EndIf 
%         \EndFor
%         \State \(\hat{\mu}_{k,t}\gets {S}_{k,t}^{\text{IE}} / {\tau}_{k,t}, \hat{\nu}_t\gets {S}_{k,t}^{\text{UE}} / {\iota}_{k,t},\,\forall k\)
%     \end{algorithmic}
% \end{algorithm}





% \subsection{Successive Accept and Reject}

% In this subsection, we illustrate how leader accepts and rejects arms in the shareable arm setting, and how all players update their information after the leader's update. 
% \setlength{\textfloatsep}{0pt}
% \begin{algorithm}[htp]
%     \caption{\(\texttt{SIC-SDA.AccRej}(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t, \mathcal{K}_t, M_t)\)}
%     \label{alg:sic_sda_accept_and_reject}
%     \begin{algorithmic}[1]
%         \State \algorithmicensure \(\mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t,\bm{m}_t^l, \bm{m}_t^u\)
%         \If{\(i=1\)}
%             \State \(\hat{\mu}_{k,t}\gets {S}_{k,t}^{\text{IE}} / {\tau}_{k,t}, \hat{\nu}_t\gets {S}_{k,t}^{\text{UE}} / {\iota}_{k,t},\,\forall k\)
%             \State Update \(\bm{m}^l_t, \bm{m}^u_t\) according to Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update})
%             \State \multiline{Update \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t\) by Eq.(\ref{eq:accept_set})(\ref{eq:reject_set})(\ref{eq:marginal_arm})}
%         \EndIf
%     \end{algorithmic}
% \end{algorithm}

% \noindent
% \textbf{Leader accepts and rejects arms.} After leader receives followers' IE observations, 
% the leader updates his empirical reward mean and check whether there are some optimal (sub-optimal) arms that should be accepted (rejected). 
% Denote \(g(k,j)\) as a special indicator function for distinguishing ``good'' arm \(k\) from ``bad'' arm \(j\) as follows
% \[g(k,j)\!\coloneqq\! \1{\hat{\mu}_{k,t}\!-\! 3\sqrt{{\log (T)}/{2\tau_{k,t}}}\! \ge\! \hat{\mu}_{j,t}\!+ \! 3\sqrt{{\log (T)}/{2\tau_{j,t}}}},\] 
% where $g(k,j) =1$ implies that the arm \(k\)'s reward mean is higher than arm \(j\)'s with high confidence.
% % For an arm \(k\), denote \(\mathcal{B}_{k,t} \coloneqq \{i\in\mathcal{K}_t: g(k,i)=0\}\) as  

% The leader accepts arm \(k\) if  the arm's resources are well estimated, i.e., \(k\in\mathcal{K}_t\setminus \mathcal{K}'_t\) and \(
%     \sum_{j\in\mathcal{K}_t: g(k,j) = 0} m_{j,t}^u \le M_t
% \), which means the total resources' upper confidence bounds 
% of arms which cannot be distinguished as bad by arm \(k\) (i.e., \(g(k,j) = 0\)) is no greater than the number of active players \(M_t\), 
% Thus, the accept arm set \(\mathcal{A}_t\) can be set as:
% \begin{equation}\label{eq:accept_set}
%     \mathcal{A}_t \coloneqq \left\{k\in\mathcal{K}_t\setminus \mathcal{K}'_t:   \sum\nolimits_{j\in\mathcal{K}_t: g(k,j) = 0}  m_{j,t}^u \le M_t\right\}. 
% \end{equation}
% The leader rejects arm \(k\), if \(
%     \sum_{j\in\mathcal{K}_t: g(j,k) = 1} m_{j,t}^l \ge M_t 
% \). 
% The inequality means that the total resources' lower confidence bounds of arms whose reward mean is higher than arm \(k\)'s with high confidence (i.e., \(g(j,k) = 1\)) is no less than \(M_t\).
% Thus, the reject arm set \(\mathcal{R}_t\) can be expressed as:
% \begin{equation}\label{eq:reject_set}
%     \mathcal{R}_t \coloneqq \left\{k\in\mathcal{K}_t: \sum\nolimits_{j\in\mathcal{K}_t: g(j,k) = 1} m_{j,t}^l \ge M_t\right\}. 
% \end{equation}
% An arm \(k\) is the empirical least favored among optimal arms if its empirical reward mean is higher than all other current active arms' with high confidence (i.e., the only optimal arm among them), and its resources' lower confidence bound is no less than \(M_t\), i.e.,
% % \(
% %     \sum_{i\in\mathcal{K}_t} g(k,i) = \abs{\mathcal{K}_t} - 1 \text{ and } m_k^l \ge M_t.
% % \)
% % The marginal accept arm \(\mathcal{L}_t\) corresponds to the worst arm among optimal arms and the ``marginal'' means the arms' capacity may only be marginally utilized.   
% \begin{equation}\label{eq:marginal_arm}
%     \mathcal{L}_t\! \coloneqq \!\left\{k\in\mathcal{K}_t \! : \!\! \sum\nolimits_{j\in\mathcal{K}_t} \! g(k,j)\! = \! K_t\! - \!1, m_{k,t}^l \!\ge\! M_t \right\}.
% \end{equation}

% \noindent
% \textbf{Players update theirs status. }
% After the leader sends back his updated information to followers, all players update their status. 
% It consists of three steps: (1) upon finding the least favored arm,
% % (line~\ref{alg:line:sic_sda_update_least_favored_arm}), 
% all active players turn to exploit this arm,
% (2) if there are accepted arms,
% % (line~\ref{alg:line:sic_sda_update_accepted_arm}), 
% several players will turn to exploit these arm, and the number of players exploiting an arm is equal to the arm's resources capacity,
% % their resources size \(m_k\) number of players turns to exploit them,
% and (3) if  \(M_t > K_t\) , update the vector \(\bm{b}_t\) to record the player allocation in the next IE round. Their details are deferred to Appendix~\ref{appsub:sic_sda_update}.


% \begin{algorithm}[htp]
%     \caption{\(\texttt{SIC-SDA.Update}(i, \mathcal{K}_t, M_t, \mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t)\)}
%     \label{alg:sic_sda_update}
%     \begin{algorithmic}[1]
%         \State \algorithmicensure \(\exparm, \mathcal{K}_t, M_t\)
%         \State \(M_t \gets M_t - \sum_{k\in\mathcal{A}_t}m_{k,t}^l\)
%         \State \(\mathcal{K}_t \gets \mathcal{K}_t\setminus (\mathcal{A}_t \cup \mathcal{R}_t \cup \mathcal{L}_t)\)

%         \If{\(\mathcal{L}_t \neq \emptyset\)}\label{alg:line:sic_sda_update_least_favored_arm}\Comment{exploit the leader favored arm}
%             \State  \(\exparm\gets \mathcal{L}_t.\)
%         \ElsIf{\(i > M_t\)}\label{alg:line:sic_sda_update_accepted_arm}\Comment{exploit accepted arm}
%             \State \multiline{\(\exparm\gets j\)-th accept arm where such that \(\sum_{n=1}^j m_{\sigma'(n),t}^l \ge i-M_t > \sum_{n=1}^{j-1} m_{\sigma'(n),t}^l\) where \(\sigma'(n)\) is the \(n\)-th accept arm.}
%         \Else 
%             \State \(\bm{b}_t\gets \bm{1}.\) \Comment{update player allocation in next IE} \label{alg:sic_sda_update:b_start}
%             \If{\(M_t > K_t\)}\label{alg:line:sic_sda_update_b} 
%                 \State \(d\gets M_t - \abs{\mathcal{K}_t}.\)
%                 \ForAll{\(k \in \mathcal{K}_t\)}
%                 \While{\(d>0\) and \(b_{k,t} < m_{k,t}^l\)}
%                     \State \(b_{k,t} \gets b_{k,t} + 1\); \(d\gets d - 1\).
%                 \EndWhile
%                 \EndFor
%             \EndIf \label{alg:sic_sda_update:b_end}
%         \EndIf
%         \State \(p\gets p + 1\)  
%     \end{algorithmic}
% \end{algorithm}

\subsection{Regret bound of \texttt{SIC-SDA}}

The following theorem states the regret upper bound for the \texttt{SIC-SDA} algorithm. Its detailed proof is in Appendix~\ref{app:sic_sda_regret}.

\begin{theorem}
    \label{thm:sic_sda_regret}
    For any given set of parameters \(K, M, \bm{\mu}, \bm{m}\), the regret of \emph{\texttt{SIC-SDA}} is upper bounded as follows:
    \begin{align}
            \ERT\! \le  & c_1\!\sum\nolimits_{k=L+1}^K \frac{M \log T}{\mu_L-\mu_k} \! +  \!c_2\!\sum\nolimits_{k=1}^M \!\frac{m_k^2}{\mu_k^2}\log T \nonumber\\
            + c_3 K^2 \log^2 & \!\left(\!\max \!\left\{\!\frac{\log (T)}{(\mu_L - \mu_{L+1})^2}, \frac{m_M^2\log(T)}{\mu_M^2} \!\right\}\!\right), \label{eq:sic_sda_regret}     
    \end{align}
    where \(c_1, c_2, c_3\) are universal positive constants. 
\end{theorem}

Eq.(\ref{eq:sic_sda_regret})'s first term corresponds to the individual exploration and successive accept and reject.
The second term is derived from the united exploration for learning resources capacities. 
The third term corresponds to the communication phase.  



% \subsection{{Synchronization Involved Communication for {Sharing Demand Information} Feedback}}
% Since the SDI's \(a_{k,t}\) feedback directly implies the SDA's \(\1{a_{k,t} > 1}\) feedback,
% the \texttt{SIC-SDA} algorithm also works under the stronger SDI feedback. 
% We name the adapted algorithm as \texttt{SIC-SDI}.


==> sections/sic_sda_algo_backup.tex <==
% !TeX root = ../decentralized_sa.tex
\section{Synchronization Involved Communication for Sharing Demand Awareness Feedback}
% Borrow as much description as possible from the previous section and try to make the structure simple and the ``improvement and adaption'' clear. 

In this section, we propose the \texttt{SIC-SDA} algorithm to tackle the more difficult SDA feedback. 
Different from observing the number of players sharing an arm, under this setting each player can only observe whether its playing arm is shared or not. 

One challenge in this weaker feedback model is that players cannot distinguish whether an arm sharing \(\1{a_{k,t} > 1}\) is for utilizing more resources of a good arm or for communication.
Not being able to differentiate them made the ad-hoc communication protocol used by \texttt{DPE-SDI} invalid. 
% We thus propose the pre-defined grid-based \texttt{SIC-SDA} algorithms.
To address that, we propose the \texttt{SIC-SDA} algorithm with phase-based communication protocol.
It consists of several phases: 
\begin{enumerate}
    \item Initialization Phase: learn \(M\) and assign ranks. 
    \item Exploration Phase: Individual and united explorations.
    \item Communication and Successive Accept and Reject: \begin{itemize}
        \item Followers send their observations forth to leader.
        \item Leader update statistics and apply the successive accept and reject procedure.
        \item Leader send his updated information back to followers.  
    \end{itemize}
    \item Exploitation Phase: player plays its assigned arms to the end. 
\end{enumerate}

% In the initialization phase, all players estimate the number of players \(M\) in the system and 
% each player is assigned with a rank from \(\{1,2,\ldots,M\}\).

% After initialization, the main structure of the \texttt{SIC-SDA} algorithm is 
% to individually and unitedly explore all candidate arms for estimating their reward means and shareable resources,
% and after a phase of explorations, followers communicate their observations to a leader,
% and the leader decides which arms to accept and which to reject and then send these information to followers. 
% Some followers will turn to exploit accepted arms, while others will continue to explore active arms until all players are in exploitation phase.
% (arms that have not been accepted or rejected).

Different from the \texttt{DPE-SDI}'s leader-follower procedure, the leader in \texttt{SIC-SDA} not only utilizes his own observations, but also uses (and receives) other followers' observations.
Because in \texttt{SIC-SDA} followers also participate in exploring sub-optimal arms.
So there are two part of communications in \texttt{SIC-SDA}: (1) leader collects follower's observations and (2) leader sends its updated information to followers.  


After each phase of exploration, some arms may be rejected as sub-optimal ones, while some may be accepted to be optimal arms and be exploited by some players. 
We call the remaining arms as \textbf{active arms}.
Denote \(\mathcal{K}_t\) as the set of active arms at time slot \(t\) and \(K_t\) as the number of active arms at time \(t\). 
Apart from players exploiting arms, the remaining players are called \textbf{active players}. 
Denote \(M_t\) as the number of active players at time slot \(t\).
% Followers maintain \(\{\mathcal{K}_t, \bm{m}^l_t, \bm{m}^u_t\}\), where \(\mathcal{K}_t\) stands for the set of \textbf{active arms} which have not been rejected or accepted and \(\bm{m}^l_t, \bm{m}^u_t\) denote the lower and upper confidence bounds of shareable resources.

\begin{algorithm}[htp]
    \caption{\texttt{SIC-SDA}}
    \label{alg:sic_sda}
    \begin{algorithmic}[1]
        \State Initialize \(\text{ExploitArm} \gets -1\); \(p\gets 1\); \(M_t \gets M\); \(\mathcal{K}_t\gets [K]\); \(\bm{S}^{\text{IE}}_t,\bm{S}_t^{\text{UE}}\gets \bm{0}, \bm{b}_t\gets \bm{1}\)
        \State \((i,M)\gets\texttt{SIC-SDA.Init()}\)
        \While{\(\text{ExploitArm} = -1\)}
            \State \multiline{\((\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t)\gets \texttt{SIC-SDA.Explore}(i, p,\bm{b}_t,\mathcal{K}_t, K_t, M_t)\)}
            
            \If{\(i=1\)}\Comment{Leader}
                \State \multiline{\((\bm{S}^{\text{IE}}_t,\bm{\tau}_t)\qquad\qquad\gets\texttt{SIC-SDA.CommBack}()\)\Comment{Receive}}
                \State \multiline{\((\mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t,\bm{m}_t^l, \bm{m}_t^u)\gets\texttt{SIC-SDA.AccRej}(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t, \mathcal{K}_t, M_t)\)} \State \(\texttt{SIC-SDA.CommForth}(\mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t,\bm{m}_t^l, \bm{m}_t^u)\)
            \ElsIf{\(i\neq 1\)}\Comment{Follower}
               \State \(\texttt{SIC-SDA.CommBack}(i, p, \bm{S}^{\text{IE}}_t)\)
               \State \multiline{\((\mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t,\bm{m}_t^l, \bm{m}_t^u)\gets\texttt{SIC-SDA.CommForth}()\) \Comment{Receive}}
            \EndIf
            
            \State \multiline{\((\text{ExploitArm}, \mathcal{K}_t, M_t, p)\gets\texttt{SIC-SDA.Update}(i, p, \mathcal{K}_t, M_t, \mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t)\)}
        \EndWhile
        \State Play the \(\text{ExploitArm}\).
    \end{algorithmic}
\end{algorithm}

\subsection{Initialization phase}

We apply the same initialization phase as DPE1~\cite{wang_optimal_2020}, whose objectives are to estimate the number of players \(M\) and to assign a rank for each player.
It consists of two sub-phases: (1) orthogonalizing players to \(K\) arms and denoting the settled arm index as its external rank; (2) assigning the internal ranks to all players according to the times of sharing awareness when these players sequentially hopping among arms. The detailed procedure is described in Appendix~\ref{appsub:sic_sa_init}.


% In initialization phase consists of two phases: orthogonalization and rank assignment. 
% The procedure is the same as~\cite{wang_optimal_2020}'s. We s

\subsection{Exploration Phase}

The exploration phase consists of two parts: individual exploration (IE) and united exploration (UE). 
While the UE part is very similar to DPE-SA's, this IE part is different.
% This is because (1) the active arms in \(\mathcal{K}_t\) of \texttt{SIC-SDA} is explored by \(M_t\) active players, while the empirical optimal arm set \(\mathcal{S}_t\) of \texttt{DPE-SDI} is explored by all \(M\) players; (2) \texttt{SIC-SDA} does not employ parsimonious exploration and all players participate the exploration.
% Since the number of active arms \(K_t\) and the number of active players \(M_t\) change as the algorithm runs, 
When individually exploring arm \(k\), the number of players \(a_{k,t}\) is unobservable under the weaker SDA feedback. 
To infer \(a_{k,t}\) in IE, players need to follow a rule: if a player's rank \(i\) is less then the number of active arms \(K_t\), he plays arm \((i+t)\Mod{K_t}\); otherwise, he choose the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n)}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n)}^l - 1)\) where \(\sigma(n)\) denotes the \(n\)-active arm among \(\mathcal{K}_t\). 
The inequality means that if an arm's rank is higher than \(K_t\), it needs to share an active arm with
others. 
That happens when the number of active players \(M_t\) is greater than \(K_t\).
% To update and record the number of players on each arm in IE,
We employ an vector \(\bm{b}\in\N^K\) to record how active arms are shared in IE. 

\begin{algorithm}
    \caption{\(\texttt{SIC-SDA.Explore}(i, p,\bm{b}_t,\mathcal{K}_t, K_t, M_t)\)}
    \begin{algorithmic}
        \State \algorithmicensure \(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t\)
        \For{\(\min\{K_t, M_t\}2^p\) times} \Comment{Individual Exploration}
            \If{\(i \le K_t\)}
                \State Play the \((i+t)\Mod{K_t}\)-th active arm.
                \State \(S^{\text{IE}}_{\pi,t}\gets S^{\text{IE}}_{\pi,t} + \frac{r_{\pi,t}}{b_{k,t}}\)
            \ElsIf{\(i > \abs{\mathcal{K}_t}\)}
                \State\multiline{Play the \(j\)-th active arm such that \(\sum_{n=1}^j (m_{\sigma(n),t}^l - 1) \ge i > \sum_{n=1}^{j-1} (m_{\sigma(n),t}^l - 1)\) where \(\sigma(n)\) denotes the \(n\)-th active arm.}
            \EndIf
        \EndFor
        \State \(\mathcal{K}'_t \gets \{k\in\mathcal{K}_t: m_{k,t}^l \neq m_{k,t}^u\}\)
        \For{\(2^p\) times} \Comment{United Exploration}
            \ForAll{ arm \(k \in \mathcal{K}'_t\)} 
                \State Play arm \(k\)
                \State \(S^{\text{UE}}_{k,t}\gets S^{\text{UE}}_{k,t} + r_{k,t}\)
            \EndFor
        \EndFor
        \State \(\hat{\mu}_{k,t}\gets {S}_{k,t}^{\text{IE}} / {\tau}_{k,t}, \hat{\nu}_t\gets {S}_{k,t}^{\text{UE}} / {\iota}_{k,t},\,\forall k\)
    \end{algorithmic}
\end{algorithm}


\subsection{Communication}
There are two kinds of communications: (1) followers send their IE accumulative reward \(\bm{S}^{\text{IE}_t}\) back to leader, (2) leader sends his updated information \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t\) forth to followers. 

\texttt{SIC-SDA.CommBack}: \emph{Followers send \(\bm{S}^{\text{IE}}\) to the leader.}
This communication utilizes the \(\1{a_{k,t} \ge 1}\) indicator feedback to transmit information.
In the \(n\)-th phase, each arm is individually explored \(2^n\) times. 
So, a follower's accumulated reward of arm \(k\) till the end of phase \(p\) is at most \(2^{p+1} - 1\) and thus can be transmitted from the follower to leader in \(p+1\) time slots via the \(\1{a_{k,t} \ge 1}\) indicator, i.e., one time slot for one bit. 
Especially, we use arm \(1\) as the communication arm.
The leader always play arm \(1\). 
When needing to send bit \(1\) to the leader, the follower plays the arm \(1\). 
This part of communication is mesh-grid: for time slots corresponding to \((j,k)\in [2, \min\{M_t, K_t\}]\times [K_t]\), follower with rank \(i = j\) will send arm \(k\)'s IE reward summation \(S^{\text{IE}}_k\) to leader. 

\begin{algorithm}
    \caption{\(\texttt{SIC-SDA.CommBack}(i, p, \bm{S}^{\text{IE}}_t)\)}
    \begin{algorithmic}
        \For{\((j,k)\in [2, \min\{M_t, K_t\}]\times [K_t]\)}
            \If{\(i=1\)}
                \State \multiline{Leader receives \(S^{\text{IE}}_{k,t}(j)\) from follower with rank \(j\) in \(p+1\) time slots.}
                \State \(S_{k,t}^{\text{IE}}(1) \gets S_{k,t}^{\text{IE}}(1) + S^{\text{IE}}_{k,t}(j)\)
                \State \(\tau_{k,t} \gets \tau_{k,t} + 2^p\)
            \ElsIf{\(i=j\)}
                \State \multiline{The follower with rank \(j\) sends \(S^{\text{IE}}_{k,t}(j)\) to leader in \(p+1\) time slots.}
            \EndIf 
        \EndFor
    \end{algorithmic}
\end{algorithm}

\texttt{SIC-SDA.CommForth}: \emph{Leader send \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t\) to followers. }
This part of communication is similar to \texttt{DPE-SDI}'s \(6\)-block procedure. 
As \texttt{SIC-SDA}'s communication is phase-based, there is no need of an initial block. 
Each block update one of \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t, \bm{m}^l_t, \bm{m}^u_t\) in \(K_t\) time slots.
The detail protocol is provided in Appendix~\ref{appsub:sic_sa_comm}




\subsection{Successive Accept and Reject}

We note that the successive accept and reject was made in~\cite{bubeck_multiple_2013} for top \(k\) arms identification and was utilized to design MMAB algorithms in~\cite{boursier_sic-mmab_2019}.
We further extend the idea to our MMAB-SA case where accepting and rejecting arms no only depends on \(K_t\)
and \(M_t\), but also each arm's among of shareable resources which are unknown a prior.

\begin{algorithm}[htp]
    \caption{\(\texttt{SIC-SDA.AccRej}(\bm{S}^{\text{IE}}_t, \bm{S}^{\text{UE}}_t, \bm{\tau}_t, \bm{\iota}_t, \mathcal{K}_t, M_t)\)}
    \label{alg:sic_sda_leader_update}
    \begin{algorithmic}[1]
        \State \algorithmicensure \(\mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t,\bm{m}_t^l, \bm{m}_t^u\)
        \If{\(i=1\)}
            \State Update \(\bm{m}^l_t, \bm{m}^u_t\) according to Eq.(\ref{eq:lower_bound_update})(\ref{eq:upper_bound_update}).
            \State \multiline{Update \(\mathcal{A}_t\), \(\mathcal{R}_t\), \(\mathcal{L}_t\) by Eq.(\ref{eq:accept_set})(\ref{eq:reject_set})(\ref{eq:marginal_arm}).}
        \EndIf
    \end{algorithmic}
\end{algorithm}

\textbf{Leader accept and reject arms.} After leader receives followers' IE observations, he updates his empirical reward mean and check whether there are some good (bad) arms that should be accepted (rejected). 
Denote \(g(k,j)\) as a special indicator function for distinguishing good arm \(k\) from bad arm \(j\) as follows
\[g(k,j)\coloneqq \1{\hat{\mu}_{k,t}- 3\sqrt{\frac{\log (T)}{2\tau_{k,t}}} \ge \hat{\mu}_{k,t} + 3\sqrt{\frac{\log (T)}{2\tau_{k,t}}}},\] 
where $g(k,j) =1$ means that arm \(k\)'s reward mean is higher than arm \(j\)'s with high confidence.
% For an arm \(k\), denote \(\mathcal{B}_{k,t} \coloneqq \{i\in\mathcal{K}_t: g(k,i)=0\}\) as  

Accept arm \(k\) if the summation of resources' upper confidence bounds of arms that arm \(k\) is not higher than with high confidence (i.e., \(g(k,j) = 0\)) is no greater than \(M_t\), i.e.,
\(
    \sum_{j\in\mathcal{K}_t: g(k,j) = 0} m_{j,t}^u \le M_t.
\) and the arm's among of resources is well estimated, i.e., \(k\in\mathcal{K}_t\setminus \mathcal{K}'_t\).
So, the accept arm set \(\mathcal{A}_t\) is 
\begin{equation}\label{eq:accept_set}
    \mathcal{A}_t \coloneqq \left\{k\in\mathcal{K}_t\setminus \mathcal{K}'_t:   \sum_{j\in\mathcal{K}_t: g(k,j) = 0}  m_{j,t}^u \le M_t\right\}. 
\end{equation}
Reject arm \(k\) if the summation of resources' lower confidence bounds of arms whose reward mean is higher than arm \(k\)'s with high confidence is no less than \(M_t\), i.e.,
\(
    \sum_{j\in\mathcal{K}_t: g(j,k) = 1} m_{j,t}^l \ge M_t.
\) and the arm's among of resources is well estimated.
So, the reject arm set \(\mathcal{R}_t\) is 
\begin{equation}\label{eq:reject_set}
    \mathcal{R}_t \coloneqq \left\{k\in\mathcal{K}_t\setminus \mathcal{K}'_t: \sum_{j\in\mathcal{K}_t: g(j,k) = 1} m_{j,t}^l \ge M_t\right\}. 
\end{equation}
An arm \(k\) is the least favored among optimal arms if its reward mean is higher than all other arms with high confidence and its resources' lower confidence bound can cover all active arms, i.e.,
% \(
%     \sum_{i\in\mathcal{K}_t} g(k,i) = \abs{\mathcal{K}_t} - 1 \text{ and } m_k^l \ge M_t.
% \)
% The marginal accept arm \(\mathcal{L}_t\) corresponds to the worst arm among optimal arms and the ``marginal'' means the arms' capacity may only be marginally utilized.   
\begin{equation}\label{eq:marginal_arm}
    \mathcal{L}_t \coloneqq \left\{k\in\mathcal{K}_t \! : \!\! \sum_{j\in\mathcal{K}_t} \! g(k,j)\! = \! K_t - 1, m_{k,t}^l \ge M_t \right\}.
\end{equation}

\textbf{Players update theirs status. }
After the leader sends back his updated information to followers, all players update their status. 
It consists of three parts: (1) if finding the least favored arm, all active players turn to exploit this arm since then,
(2) if there are accepted arms, assign its resources size \(m_k\) number of players to exploit them,
and (3) if  \(M_t > K_t\), update the vector \(\bm{b}_t\) to record the player allocation in IE.

\begin{algorithm}[htp]
    \caption{\(\texttt{SIC-SDA.Update}(i, \mathcal{K}_t, M_t, \mathcal{A}_t, \mathcal{R}_t, \mathcal{L}_t)\)}
    \label{alg:sic_sda_update}
    \begin{algorithmic}[1]
        \State \algorithmicensure \(\text{ExploitArm}, \mathcal{K}_t, M_t\)
        \State \(M_t \gets M_t - \sum_{k\in\mathcal{A}_t}m_{k,t}^l\)
        \State \(\mathcal{K}_t \gets \mathcal{K}_t\setminus (\mathcal{A}_t \cup \mathcal{R}_t \cup \mathcal{L}_t)\)

        \If{\(\mathcal{L}_t \neq \emptyset\)}
            \State  \(\text{ExploitArm}\gets \mathcal{L}_t.\)
        \ElsIf{\(i > M_t\)}
            \State \multiline{\(\text{ExploitArm}\gets j\)-th accept arm where such that \(\sum_{n=1}^j m_{\sigma'(n),t}^l \ge i-M_t > \sum_{n=1}^{j-1} m_{\sigma'(n),t}^l\) where \(\sigma'(n)\) is the \(n\)-th accept arm.}
        \Else 
            \State \(\bm{b}_t\gets \bm{1}.\)
            \If{\(M_t > K_t\)}
                \State \(d\gets M_t - \abs{\mathcal{K}_t}.\)
                \ForAll{\(k \in \mathcal{K}_t\)}
                \While{\(d>0\) and \(b_{k,t} < m_{k,t}^l\)}
                    \State \(b_{k,t} \gets b_{k,t} + 1\); \(d\gets d - 1\).
                \EndWhile
                \EndFor
            \EndIf
        \EndIf
        \State \(p\gets p + 1\)  
    \end{algorithmic}
\end{algorithm}


\subsection{{Synchronization Involved Communication for \emph{Sharing Information} Feedback}}
Since the SDI's \(a_{k,t}\) feedback directly implies the SDA's \(\1{a_{k,t} > 1}\) feedback,
the \texttt{SIC-SDA} algorithm also works under the stronger SDI feedback. 
We name the adapted algorithm as \texttt{SIC-SDI}.
